Do VLMs Need to Keep Looking at Long Videos? Write It Down, Then Look Away

Vision-language models (VLMs) reason about long videos over hundreds to thousands of tokens. Every decoding step re-reads the key-value (KV) cache of the entire video. Must the model keep looking while it reasons? In LookAway, the model first writes timestamped notes on what the question needs and then puts the video away. Once the notes close, the inference engine hides the video's KV cache for the rest of the response. Across both hybrid and pure-attention VLMs, dependence on the video is concentrated early in the response. On Qwen3.6-27B, writing notes preserves accuracy better than free reasoning at the same withdrawal step. Replacing them with another video's notes harms accuracy, whereas keeping the video visible alongside the model's own notes adds no significant benefit. Without additional training, LookAway nearly matches full-video thinking accuracy at 0.12-0.13 times its modeled decode cost. To shorten this initial look, we fine-tune the model on its own correct LookAway responses. Reinforcement learning then rewards correct answers while penalizing KV reads. The trained model puts the video away after a median of 66-68 tokens. Across three held-out benchmarks, it writes more tokens than an identically trained full-video model yet reads only 27-35% as many KV positions at matched accuracy.

==> numbers.tex <==
% Generated by tools/paper_numbers.py. Do not edit by hand.
\makeatletter
\expandafter\def\csname N@bd.mmmu.bf.tmax\endcsname{0.52}
\expandafter\def\csname N@bd.mmmu.bf.tmin\endcsname{0.39}
\expandafter\def\csname N@bd.mmmu.bf1024.acc\endcsname{86.2}
\expandafter\def\csname N@bd.mmmu.bf1024.d\endcsname{+0.5}
\expandafter\def\csname N@bd.mmmu.bf1024.d.abs\endcsname{0.5}
\expandafter\def\csname N@bd.mmmu.bf1024.d.ci\endcsname{[$-$1.7, +2.7]}
\expandafter\def\csname N@bd.mmmu.bf1024.d.hi\endcsname{+2.7}
\expandafter\def\csname N@bd.mmmu.bf1024.d.lo\endcsname{$-$1.7}
\expandafter\def\csname N@bd.mmmu.bf1024.t\endcsname{0.52}
\expandafter\def\csname N@bd.mmmu.bf1024.t.ci\endcsname{[0.44, 0.61]}
\expandafter\def\csname N@bd.mmmu.bf1024.t.pct\endcsname{52.2}
\expandafter\def\csname N@bd.mmmu.bf1024.tok\endcsname{1,779}
\expandafter\def\csname N@bd.mmmu.bf256.acc\endcsname{83.5}
\expandafter\def\csname N@bd.mmmu.bf256.d\endcsname{$-$2.3}
\expandafter\def\csname N@bd.mmmu.bf256.d.abs\endcsname{2.3}
\expandafter\def\csname N@bd.mmmu.bf256.d.ci\endcsname{[$-$5.0, +0.3]}
\expandafter\def\csname N@bd.mmmu.bf256.d.hi\endcsname{+0.3}
\expandafter\def\csname N@bd.mmmu.bf256.d.lo\endcsname{$-$5.0}
\expandafter\def\csname N@bd.mmmu.bf256.t\endcsname{0.39}
\expandafter\def\csname N@bd.mmmu.bf256.t.ci\endcsname{[0.32, 0.47]}
\expandafter\def\csname N@bd.mmmu.bf256.t.pct\endcsname{38.7}
\expandafter\def\csname N@bd.mmmu.bf256.tok\endcsname{1,349}
\expandafter\def\csname N@bd.mmmu.bf256.vsnotes\endcsname{2.9}
\expandafter\def\csname N@bd.mmmu.bf512.acc\endcsname{84.5}
\expandafter\def\csname N@bd.mmmu.bf512.d\endcsname{$-$1.3}
\expandafter\def\csname N@bd.mmmu.bf512.d.abs\endcsname{1.3}
\expandafter\def\csname N@bd.mmmu.bf512.d.ci\endcsname{[$-$3.8, +1.2]}
\expandafter\def\csname N@bd.mmmu.bf512.d.hi\endcsname{+1.2}
\expandafter\def\csname N@bd.mmmu.bf512.d.lo\endcsname{$-$3.8}
\expandafter\def\csname N@bd.mmmu.bf512.t\endcsname{0.44}
\expandafter\def\csname N@bd.mmmu.bf512.t.ci\endcsname{[0.37, 0.52]}
\expandafter\def\csname N@bd.mmmu.bf512.t.pct\endcsname{44.0}
\expandafter\def\csname N@bd.mmmu.bf512.tok\endcsname{1,544}
\expandafter\def\csname N@bd.mmmu.wd128.acc\endcsname{75.8}
\expandafter\def\csname N@bd.mmmu.wd128.d\endcsname{$-$10.0}
\expandafter\def\csname N@bd.mmmu.wd128.d.abs\endcsname{10.0}
\expandafter\def\csname N@bd.mmmu.wd128.d.ci\endcsname{[$-$14.3, $-$6.0]}
\expandafter\def\csname N@bd.mmmu.wd128.d.hi\endcsname{$-$6.0}
\expandafter\def\csname N@bd.mmmu.wd128.d.lo\endcsname{$-$14.3}
\expandafter\def\csname N@bd.mmmu.wd128.t\endcsname{0.23}
\expandafter\def\csname N@bd.mmmu.wd128.t.ci\endcsname{[0.19, 0.29]}
\expandafter\def\csname N@bd.mmmu.wd128.t.pct\endcsname{23.2}
\expandafter\def\csname N@bd.mmmu.wd128.tok\endcsname{4,517}
\expandafter\def\csname N@bd.mmmu.wd256.acc\endcsname{80.8}
\expandafter\def\csname N@bd.mmmu.wd256.d\endcsname{$-$5.0}
\expandafter\def\csname N@bd.mmmu.wd256.d.abs\endcsname{5.0}
\expandafter\def\csname N@bd.mmmu.wd256.d.ci\endcsname{[$-$8.3, $-$2.0]}
\expandafter\def\csname N@bd.mmmu.wd256.d.hi\endcsname{$-$2.0}
\expandafter\def\csname N@bd.mmmu.wd256.d.lo\endcsname{$-$8.3}
\expandafter\def\csname N@bd.mmmu.wd256.t\endcsname{0.22}
\expandafter\def\csname N@bd.mmmu.wd256.t.ci\endcsname{[0.20, 0.25]}
\expandafter\def\csname N@bd.mmmu.wd256.t.pct\endcsname{21.9}
\expandafter\def\csname N@bd.mmmu.wd256.tok\endcsname{3,798}
\expandafter\def\csname N@bd.mmmu.wd64.acc\endcsname{71.5}
\expandafter\def\csname N@bd.mmmu.wd64.d\endcsname{$-$14.3}
\expandafter\def\csname N@bd.mmmu.wd64.d.abs\endcsname{14.3}
\expandafter\def\csname N@bd.mmmu.wd64.d.ci\endcsname{[$-$19.5, $-$9.2]}
\expandafter\def\csname N@bd.mmmu.wd64.d.hi\endcsname{$-$9.2}
\expandafter\def\csname N@bd.mmmu.wd64.d.lo\endcsname{$-$19.5}
\expandafter\def\csname N@bd.mmmu.wd64.t\endcsname{0.26}
\expandafter\def\csname N@bd.mmmu.wd64.t.ci\endcsname{[0.21, 0.32]}
\expandafter\def\csname N@bd.mmmu.wd64.t.pct\endcsname{25.9}
\expandafter\def\csname N@bd.mmmu.wd64.tok\endcsname{5,344}
\expandafter\def\csname N@bd.vh.bf.tmax\endcsname{0.43}
\expandafter\def\csname N@bd.vh.bf.tmin\endcsname{0.29}
\expandafter\def\csname N@bd.vh.bf1024.acc\endcsname{70.5}
\expandafter\def\csname N@bd.vh.bf1024.d\endcsname{$-$0.8}
\expandafter\def\csname N@bd.vh.bf1024.d.abs\endcsname{0.8}
\expandafter\def\csname N@bd.vh.bf1024.d.ci\endcsname{[$-$3.0, +1.2]}
\expandafter\def\csname N@bd.vh.bf1024.d.hi\endcsname{+1.2}
\expandafter\def\csname N@bd.vh.bf1024.d.lo\endcsname{$-$3.0}
\expandafter\def\csname N@bd.vh.bf1024.t\endcsname{0.43}
\expandafter\def\csname N@bd.vh.bf1024.t.ci\endcsname{[0.41, 0.46]}
\expandafter\def\csname N@bd.vh.bf1024.t.pct\endcsname{43.1}
\expandafter\def\csname N@bd.vh.bf1024.tok\endcsname{1,423}
\expandafter\def\csname N@bd.vh.bf256.acc\endcsname{71.1}
\expandafter\def\csname N@bd.vh.bf256.d\endcsname{$-$0.2}
\expandafter\def\csname N@bd.vh.bf256.d.abs\endcsname{0.2}
\expandafter\def\csname N@bd.vh.bf256.d.ci\endcsname{[$-$2.5, +2.0]}
\expandafter\def\csname N@bd.vh.bf256.d.hi\endcsname{+2.0}
\expandafter\def\csname N@bd.vh.bf256.d.lo\endcsname{$-$2.5}
\expandafter\def\csname N@bd.vh.bf256.t\endcsname{0.29}
\expandafter\def\csname N@bd.vh.bf256.t.ci\endcsname{[0.26, 0.32]}
\expandafter\def\csname N@bd.vh.bf256.t.pct\endcsname{28.9}
\expandafter\def\csname N@bd.vh.bf256.tok\endcsname{946}
\expandafter\def\csname N@bd.vh.bf256.vsnotes\endcsname{2.5}
\expandafter\def\csname N@bd.vh.bf512.acc\endcsname{70.7}
\expandafter\def\csname N@bd.vh.bf512.d\endcsname{$-$0.7}
\expandafter\def\csname N@bd.vh.bf512.d.abs\endcsname{0.7}
\expandafter\def\csname N@bd.vh.bf512.d.ci\endcsname{[$-$2.6, +1.2]}
\expandafter\def\csname N@bd.vh.bf512.d.hi\endcsname{+1.2}
\expandafter\def\csname N@bd.vh.bf512.d.lo\endcsname{$-$2.6}
\expandafter\def\csname N@bd.vh.bf512.t\endcsname{0.33}
\expandafter\def\csname N@bd.vh.bf512.t.ci\endcsname{[0.30, 0.36]}
\expandafter\def\csname N@bd.vh.bf512.t.pct\endcsname{33.1}
\expandafter\def\csname N@bd.vh.bf512.tok\endcsname{1,091}
\expandafter\def\csname N@bd.vh.wd128.acc\endcsname{68.1}
\expandafter\def\csname N@bd.vh.wd128.d\endcsname{$-$3.3}
\expandafter\def\csname N@bd.vh.wd128.d.abs\endcsname{3.3}
\expandafter\def\csname N@bd.vh.wd128.d.ci\endcsname{[$-$5.7, $-$0.8]}
\expandafter\def\csname N@bd.vh.wd128.d.hi\endcsname{$-$0.8}
\expandafter\def\csname N@bd.vh.wd128.d.lo\endcsname{$-$5.7}
\expandafter\def\csname N@bd.vh.wd128.t\endcsname{0.18}
\expandafter\def\csname N@bd.vh.wd128.t.ci\endcsname{[0.17, 0.20]}
\expandafter\def\csname N@bd.vh.wd128.t.pct\endcsname{18.4}
\expandafter\def\csname N@bd.vh.wd128.tok\endcsname{2,728}
\expandafter\def\csname N@bd.vh.wd256.acc\endcsname{67.9}
\expandafter\def\csname N@bd.vh.wd256.d\endcsname{$-$3.4}
\expandafter\def\csname N@bd.vh.wd256.d.abs\endcsname{3.4}
\expandafter\def\csname N@bd.vh.wd256.d.ci\endcsname{[$-$5.6, $-$1.2]}
\expandafter\def\csname N@bd.vh.wd256.d.hi\endcsname{$-$1.2}
\expandafter\def\csname N@bd.vh.wd256.d.lo\endcsname{$-$5.6}
\expandafter\def\csname N@bd.vh.wd256.t\endcsname{0.23}
\expandafter\def\csname N@bd.vh.wd256.t.ci\endcsname{[0.21, 0.25]}
\expandafter\def\csname N@bd.vh.wd256.t.pct\endcsname{22.9}
\expandafter\def\csname N@bd.vh.wd256.tok\endcsname{2,887}
\expandafter\def\csname N@bd.vh.wd64.acc\endcsname{66.7}
\expandafter\def\csname N@bd.vh.wd64.d\endcsname{$-$4.6}
\expandafter\def\csname N@bd.vh.wd64.d.abs\endcsname{4.6}
\expandafter\def\csname N@bd.vh.wd64.d.ci\endcsname{[$-$7.3, $-$2.0]}
\expandafter\def\csname N@bd.vh.wd64.d.hi\endcsname{$-$2.0}
\expandafter\def\csname N@bd.vh.wd64.d.lo\endcsname{$-$7.3}
\expandafter\def\csname N@bd.vh.wd64.t\endcsname{0.16}
\expandafter\def\csname N@bd.vh.wd64.t.ci\endcsname{[0.15, 0.18]}
\expandafter\def\csname N@bd.vh.wd64.t.pct\endcsname{16.3}
\expandafter\def\csname N@bd.vh.wd64.tok\endcsname{2,572}
\expandafter\def\csname N@dev.basenotes.correct\endcsname{465}
\expandafter\def\csname N@dev.basenotes.t\endcsname{0.125}
\expandafter\def\csname N@dev.basevan.correct\endcsname{483}
\expandafter\def\csname N@dev.n\endcsname{661}
\expandafter\def\csname N@dev.rlnotess100.correct\endcsname{470}
\expandafter\def\csname N@dev.rlnotess100.t\endcsname{0.062}
\expandafter\def\csname N@dev.rlnotess150.correct\endcsname{489}
\expandafter\def\csname N@dev.rlnotess150.t\endcsname{0.042}
\expandafter\def\csname N@dev.rlnotess50.correct\endcsname{465}
\expandafter\def\csname N@dev.rlnotess50.t\endcsname{0.097}
\expandafter\def\csname N@dev.rlvanillas50.correct\endcsname{473}
\expandafter\def\csname N@dev.rlvanillas50.t\endcsname{0.172}
\expandafter\def\csname N@dev.sftnotes.correct\endcsname{454}
\expandafter\def\csname N@dev.sftnotes.t\endcsname{0.133}
\expandafter\def\csname N@dev.sftvanilla.correct\endcsname{458}
\expandafter\def\csname N@dev.sftvanilla.t\endcsname{0.933}
\expandafter\def\csname N@e1.mmmu.blind.acc\endcsname{69.0}
\expandafter\def\csname N@e1.mmmu.blind.hidden\endcsname{28}
\expandafter\def\csname N@e1.mmmu.blind.t\endcsname{0.18}
\expandafter\def\csname N@e1.mmmu.blind.t.ci\endcsname{[0.14, 0.23]}
\expandafter\def\csname N@e1.mmmu.blind.t.pct\endcsname{17.9}
\expandafter\def\csname N@e1.mmmu.blind.tok\endcsname{4,073}
\expandafter\def\csname N@e1.mmmu.blindloss\endcsname{16.8}
\expandafter\def\csname N@e1.mmmu.fixed-512-blind\endcsname{+16.8}
\expandafter\def\csname N@e1.mmmu.fixed-512-blind.abs\endcsname{16.8}
\expandafter\def\csname N@e1.mmmu.fixed-512-blind.ci\endcsname{[+11.3, +22.3]}
\expandafter\def\csname N@e1.mmmu.fixed-512-blind.hi\endcsname{+22.3}
\expandafter\def\csname N@e1.mmmu.fixed-512-blind.lo\endcsname{+11.3}
\expandafter\def\csname N@e1.mmmu.fixed.acc\endcsname{85.8}
\expandafter\def\csname N@e1.mmmu.fixed.hidden\endcsname{512}
\expandafter\def\csname N@e1.mmmu.fixed.t\endcsname{0.26}
\expandafter\def\csname N@e1.mmmu.fixed.t.ci\endcsname{[0.23, 0.29]}
\expandafter\def\csname N@e1.mmmu.fixed.t.pct\endcsname{25.9}
\expandafter\def\csname N@e1.mmmu.fixed.tok\endcsname{3,343}
\expandafter\def\csname N@e1.mmmu.fixed.tratio\endcsname{2.0}
\expandafter\def\csname N@e1.mmmu.gap.fixed\endcsname{100}
\expandafter\def\csname N@e1.mmmu.gap.notes\endcsname{85}
\expandafter\def\csname N@e1.mmmu.gap.notesvis\endcsname{93}
\expandafter\def\csname N@e1.mmmu.gap.pinsonly\endcsname{57}
\expandafter\def\csname N@e1.mmmu.gap.posmatch\endcsname{73}
\expandafter\def\csname N@e1.mmmu.notes-blind\endcsname{+14.3}
\expandafter\def\csname N@e1.mmmu.notes-blind.abs\endcsname{14.3}
\expandafter\def\csname N@e1.mmmu.notes-blind.ci\endcsname{[+8.8, +20.0]}
\expandafter\def\csname N@e1.mmmu.notes-blind.hi\endcsname{+20.0}
\expandafter\def\csname N@e1.mmmu.notes-blind.lo\endcsname{+8.8}
\expandafter\def\csname N@e1.mmmu.notes-fixed-512\endcsname{$-$2.5}
\expandafter\def\csname N@e1.mmmu.notes-fixed-512.abs\endcsname{2.5}
\expandafter\def\csname N@e1.mmmu.notes-fixed-512.ci\endcsname{[$-$5.0, 0.0]}
\expandafter\def\csname N@e1.mmmu.notes-fixed-512.hi\endcsname{0.0}
\expandafter\def\csname N@e1.mmmu.notes-fixed-512.lo\endcsname{$-$5.0}
\expandafter\def\csname N@e1.mmmu.notes-visible-notes\endcsname{+1.2}
\expandafter\def\csname N@e1.mmmu.notes-visible-notes.abs\endcsname{1.2}
\expandafter\def\csname N@e1.mmmu.notes-visible-notes.ci\endcsname{[$-$1.3, +4.0]}
\expandafter\def\csname N@e1.mmmu.notes-visible-notes.hi\endcsname{+4.0}
\expandafter\def\csname N@e1.mmmu.notes-visible-notes.lo\endcsname{$-$1.3}
\expandafter\def\csname N@e1.mmmu.notes-visible-vanilla\endcsname{$-$1.3}
\expandafter\def\csname N@e1.mmmu.notes-visible-vanilla.abs\endcsname{1.3}
\expandafter\def\csname N@e1.mmmu.notes-visible-vanilla.ci\endcsname{[$-$3.3, +1.0]}
\expandafter\def\csname N@e1.mmmu.notes-visible-vanilla.hi\endcsname{+1.0}
\expandafter\def\csname N@e1.mmmu.notes-visible-vanilla.lo\endcsname{$-$3.3}
\expandafter\def\csname N@e1.mmmu.notes.acc\endcsname{83.2}
\expandafter\def\csname N@e1.mmmu.notes.chars\endcsname{430}
\expandafter\def\csname N@e1.mmmu.notes.hidden\endcsname{169}
\expandafter\def\csname N@e1.mmmu.notes.t\endcsname{0.13}
\expandafter\def\csname N@e1.mmmu.notes.t.ci\endcsname{[0.12, 0.16]}
\expandafter\def\csname N@e1.mmmu.notes.t.pct\endcsname{13.3}
\expandafter\def\csname N@e1.mmmu.notes.tok\endcsname{2,025}
\expandafter\def\csname N@e1.mmmu.notesvis.acc\endcsname{84.5}
\expandafter\def\csname N@e1.mmmu.notesvis.hidden\endcsname{171}
\expandafter\def\csname N@e1.mmmu.notesvis.t\endcsname{0.62}
\expandafter\def\csname N@e1.mmmu.notesvis.t.ci\endcsname{[0.57, 0.67]}
\expandafter\def\csname N@e1.mmmu.notesvis.t.pct\endcsname{61.9}
\expandafter\def\csname N@e1.mmmu.notesvis.tok\endcsname{2,132}
\expandafter\def\csname N@e1.mmmu.notesvis.tratio\endcsname{4.7}
\expandafter\def\csname N@e1.mmmu.nothink.acc\endcsname{84.2}
\expandafter\def\csname N@e1.mmmu.nothink.t\endcsname{0.22}
\expandafter\def\csname N@e1.mmmu.nothink.t.ci\endcsname{[0.19, 0.25]}
\expandafter\def\csname N@e1.mmmu.nothink.t.pct\endcsname{21.8}
\expandafter\def\csname N@e1.mmmu.nothink.tok\endcsname{774}
\expandafter\def\csname N@e1.mmmu.pinsonly.acc\endcsname{78.5}
\expandafter\def\csname N@e1.mmmu.pinsonly.hidden\endcsname{46}
\expandafter\def\csname N@e1.mmmu.pinsonly.t\endcsname{0.21}
\expandafter\def\csname N@e1.mmmu.pinsonly.t.ci\endcsname{[0.17, 0.25]}
\expandafter\def\csname N@e1.mmmu.pinsonly.t.pct\endcsname{20.5}
\expandafter\def\csname N@e1.mmmu.pinsonly.tok\endcsname{3,364}
\expandafter\def\csname N@e1.mmmu.position-matched-blind\endcsname{+12.3}
\expandafter\def\csname N@e1.mmmu.position-matched-blind.abs\endcsname{12.3}
\expandafter\def\csname N@e1.mmmu.position-matched-blind.ci\endcsname{[+7.3, +17.0]}
\expandafter\def\csname N@e1.mmmu.position-matched-blind.hi\endcsname{+17.0}
\expandafter\def\csname N@e1.mmmu.position-matched-blind.lo\endcsname{+7.3}
\expandafter\def\csname N@e1.mmmu.posmatch.acc\endcsname{81.2}
\expandafter\def\csname N@e1.mmmu.posmatch.hidden\endcsname{172}
\expandafter\def\csname N@e1.mmmu.posmatch.t\endcsname{0.23}
\expandafter\def\csname N@e1.mmmu.posmatch.t.ci\endcsname{[0.19, 0.27]}
\expandafter\def\csname N@e1.mmmu.posmatch.t.pct\endcsname{22.7}
\expandafter\def\csname N@e1.mmmu.posmatch.tok\endcsname{4,203}
\expandafter\def\csname N@e1.mmmu.posmatch.tokratio\endcsname{2.1}
\expandafter\def\csname N@e1.mmmu.posmatchloss\endcsname{4.5}
\expandafter\def\csname N@e1.mmmu.primary\endcsname{+2.0}
\expandafter\def\csname N@e1.mmmu.primary.abs\endcsname{2.0}
\expandafter\def\csname N@e1.mmmu.primary.ci\endcsname{[$-$2.0, +6.0]}
\expandafter\def\csname N@e1.mmmu.primary.hi\endcsname{+6.0}
\expandafter\def\csname N@e1.mmmu.primary.lo\endcsname{$-$2.0}
\expandafter\def\csname N@e1.mmmu.vanilla.acc\endcsname{85.8}
\expandafter\def\csname N@e1.mmmu.vanilla.t\endcsname{1.00}
\expandafter\def\csname N@e1.mmmu.vanilla.t.ci\endcsname{[1.00, 1.00]}
\expandafter\def\csname N@e1.mmmu.vanilla.t.pct\endcsname{100.0}
\expandafter\def\csname N@e1.mmmu.vanilla.tok\endcsname{3,425}
\expandafter\def\csname N@e1.vh.blind.acc\endcsname{65.3}
\expandafter\def\csname N@e1.vh.blind.hidden\endcsname{28}
\expandafter\def\csname N@e1.vh.blind.t\endcsname{0.13}
\expandafter\def\csname N@e1.vh.blind.t.ci\endcsname{[0.11, 0.16]}
\expandafter\def\csname N@e1.vh.blind.t.pct\endcsname{13.3}
\expandafter\def\csname N@e1.vh.blind.tok\endcsname{1,858}
\expandafter\def\csname N@e1.vh.blindloss\endcsname{6.1}
\expandafter\def\csname N@e1.vh.fixed-512-blind\endcsname{+6.4}
\expandafter\def\csname N@e1.vh.fixed-512-blind.abs\endcsname{6.4}
\expandafter\def\csname N@e1.vh.fixed-512-blind.ci\endcsname{[+3.3, +9.6]}
\expandafter\def\csname N@e1.vh.fixed-512-blind.hi\endcsname{+9.6}
\expandafter\def\csname N@e1.vh.fixed-512-blind.lo\endcsname{+3.3}
\expandafter\def\csname N@e1.vh.fixed.acc\endcsname{71.7}
\expandafter\def\csname N@e1.vh.fixed.hidden\endcsname{512}
\expandafter\def\csname N@e1.vh.fixed.t\endcsname{0.29}
\expandafter\def\csname N@e1.vh.fixed.t.ci\endcsname{[0.28, 0.31]}
\expandafter\def\csname N@e1.vh.fixed.t.pct\endcsname{29.4}
\expandafter\def\csname N@e1.vh.fixed.tok\endcsname{2,877}
\expandafter\def\csname N@e1.vh.fixed.tratio\endcsname{2.5}
\expandafter\def\csname N@e1.vh.gap.fixed\endcsname{106}
\expandafter\def\csname N@e1.vh.gap.notes\endcsname{93}
\expandafter\def\csname N@e1.vh.gap.notesvis\endcsname{75}
\expandafter\def\csname N@e1.vh.gap.pinsonly\endcsname{27}
\expandafter\def\csname N@e1.vh.gap.posmatch\endcsname{30}
\expandafter\def\csname N@e1.vh.notes-blind\endcsname{+5.6}
\expandafter\def\csname N@e1.vh.notes-blind.abs\endcsname{5.6}
\expandafter\def\csname N@e1.vh.notes-blind.ci\endcsname{[+2.9, +8.3]}
\expandafter\def\csname N@e1.vh.notes-blind.hi\endcsname{+8.3}
\expandafter\def\csname N@e1.vh.notes-blind.lo\endcsname{+2.9}
\expandafter\def\csname N@e1.vh.notes-fixed-512\endcsname{$-$0.8}
\expandafter\def\csname N@e1.vh.notes-fixed-512.abs\endcsname{0.8}
\expandafter\def\csname N@e1.vh.notes-fixed-512.ci\endcsname{[$-$3.2, +1.6]}
\expandafter\def\csname N@e1.vh.notes-fixed-512.hi\endcsname{+1.6}
\expandafter\def\csname N@e1.vh.notes-fixed-512.lo\endcsname{$-$3.2}
\expandafter\def\csname N@e1.vh.notes-visible-notes\endcsname{$-$1.1}
\expandafter\def\csname N@e1.vh.notes-visible-notes.abs\endcsname{1.1}
\expandafter\def\csname N@e1.vh.notes-visible-notes.ci\endcsname{[$-$3.3, +1.1]}
\expandafter\def\csname N@e1.vh.notes-visible-notes.hi\endcsname{+1.1}
\expandafter\def\csname N@e1.vh.notes-visible-notes.lo\endcsname{$-$3.3}
\expandafter\def\csname N@e1.vh.notes-visible-vanilla\endcsname{$-$1.5}
\expandafter\def\csname N@e1.vh.notes-visible-vanilla.abs\endcsname{1.5}
\expandafter\def\csname N@e1.vh.notes-visible-vanilla.ci\endcsname{[$-$3.8, +0.7]}
\expandafter\def\csname N@e1.vh.notes-visible-vanilla.hi\endcsname{+0.7}
\expandafter\def\csname N@e1.vh.notes-visible-vanilla.lo\endcsname{$-$3.8}
\expandafter\def\csname N@e1.vh.notes.acc\endcsname{70.9}
\expandafter\def\csname N@e1.vh.notes.chars\endcsname{566}
\expandafter\def\csname N@e1.vh.notes.hidden\endcsname{200}
\expandafter\def\csname N@e1.vh.notes.t\endcsname{0.12}
\expandafter\def\csname N@e1.vh.notes.t.ci\endcsname{[0.11, 0.13]}
\expandafter\def\csname N@e1.vh.notes.t.pct\endcsname{11.8}
\expandafter\def\csname N@e1.vh.notes.tok\endcsname{1,199}
\expandafter\def\csname N@e1.vh.notesvis.acc\endcsname{69.8}
\expandafter\def\csname N@e1.vh.notesvis.hidden\endcsname{201}
\expandafter\def\csname N@e1.vh.notesvis.t\endcsname{0.50}
\expandafter\def\csname N@e1.vh.notesvis.t.ci\endcsname{[0.47, 0.54]}
\expandafter\def\csname N@e1.vh.notesvis.t.pct\endcsname{50.4}
\expandafter\def\csname N@e1.vh.notesvis.tok\endcsname{1,596}
\expandafter\def\csname N@e1.vh.notesvis.tratio\endcsname{4.3}
\expandafter\def\csname N@e1.vh.nothink.acc\endcsname{71.0}
\expandafter\def\csname N@e1.vh.nothink.t\endcsname{0.095}
\expandafter\def\csname N@e1.vh.nothink.t.ci\endcsname{[0.088, 0.102]}
\expandafter\def\csname N@e1.vh.nothink.t.pct\endcsname{9.5}
\expandafter\def\csname N@e1.vh.nothink.tok\endcsname{323}
\expandafter\def\csname N@e1.vh.pinsonly.acc\endcsname{66.9}
\expandafter\def\csname N@e1.vh.pinsonly.hidden\endcsname{49}
\expandafter\def\csname N@e1.vh.pinsonly.t\endcsname{0.24}
\expandafter\def\csname N@e1.vh.pinsonly.t.ci\endcsname{[0.22, 0.27]}
\expandafter\def\csname N@e1.vh.pinsonly.t.pct\endcsname{24.3}
\expandafter\def\csname N@e1.vh.pinsonly.tok\endcsname{2,407}
\expandafter\def\csname N@e1.vh.position-matched-blind\endcsname{+1.8}
\expandafter\def\csname N@e1.vh.position-matched-blind.abs\endcsname{1.8}
\expandafter\def\csname N@e1.vh.position-matched-blind.ci\endcsname{[$-$0.9, +4.6]}
\expandafter\def\csname N@e1.vh.position-matched-blind.hi\endcsname{+4.6}
\expandafter\def\csname N@e1.vh.position-matched-blind.lo\endcsname{$-$0.9}
\expandafter\def\csname N@e1.vh.posmatch.acc\endcsname{67.1}
\expandafter\def\csname N@e1.vh.posmatch.hidden\endcsname{209}
\expandafter\def\csname N@e1.vh.posmatch.t\endcsname{0.21}
\expandafter\def\csname N@e1.vh.posmatch.t.ci\endcsname{[0.19, 0.23]}
\expandafter\def\csname N@e1.vh.posmatch.t.pct\endcsname{21.0}
\expandafter\def\csname N@e1.vh.posmatch.tok\endcsname{2,709}
\expandafter\def\csname N@e1.vh.posmatch.tokratio\endcsname{2.3}
\expandafter\def\csname N@e1.vh.posmatchloss\endcsname{4.2}
\expandafter\def\csname N@e1.vh.primary\endcsname{+3.8}
\expandafter\def\csname N@e1.vh.primary.abs\endcsname{3.8}
\expandafter\def\csname N@e1.vh.primary.ci\endcsname{[+1.3, +6.2]}
\expandafter\def\csname N@e1.vh.primary.hi\endcsname{+6.2}
\expandafter\def\csname N@e1.vh.primary.lo\endcsname{+1.3}
\expandafter\def\csname N@e1.vh.vanilla.acc\endcsname{71.3}
\expandafter\def\csname N@e1.vh.vanilla.t\endcsname{1.00}
\expandafter\def\csname N@e1.vh.vanilla.t.ci\endcsname{[1.00, 1.00]}
\expandafter\def\csname N@e1.vh.vanilla.t.pct\endcsname{100.0}
\expandafter\def\csname N@e1.vh.vanilla.tok\endcsname{3,162}
\expandafter\def\csname N@e2.mmmu.blind-textempty\endcsname{+11.2}
\expandafter\def\csname N@e2.mmmu.blind-textempty.abs\endcsname{11.2}
\expandafter\def\csname N@e2.mmmu.blind-textempty.ci\endcsname{[+5.8, +16.8]}
\expandafter\def\csname N@e2.mmmu.blind-textempty.hi\endcsname{+16.8}
\expandafter\def\csname N@e2.mmmu.blind-textempty.lo\endcsname{+5.8}
\expandafter\def\csname N@e2.mmmu.own.acc\endcsname{83.0}
\expandafter\def\csname N@e2.mmmu.own.prompt\endcsname{76,749}
\expandafter\def\csname N@e2.mmmu.own.t\endcsname{0.13}
\expandafter\def\csname N@e2.mmmu.own.t.ci\endcsname{[0.11, 0.14]}
\expandafter\def\csname N@e2.mmmu.own.t.pct\endcsname{12.5}
\expandafter\def\csname N@e2.mmmu.own.tok\endcsname{2,043}
\expandafter\def\csname N@e2.mmmu.reading\endcsname{inconclusive}
\expandafter\def\csname N@e2.mmmu.textempty.acc\endcsname{57.8}
\expandafter\def\csname N@e2.mmmu.textempty.prompt\endcsname{761}
\expandafter\def\csname N@e2.mmmu.textempty.t\endcsname{0.14}
\expandafter\def\csname N@e2.mmmu.textempty.t.ci\endcsname{[0.11, 0.19]}
\expandafter\def\csname N@e2.mmmu.textempty.t.pct\endcsname{14.4}
\expandafter\def\csname N@e2.mmmu.textempty.tok\endcsname{3,893}
\expandafter\def\csname N@e2.mmmu.textown-notes\endcsname{$-$3.5}
\expandafter\def\csname N@e2.mmmu.textown-notes.abs\endcsname{3.5}
\expandafter\def\csname N@e2.mmmu.textown-notes.ci\endcsname{[$-$6.8, $-$0.5]}
\expandafter\def\csname N@e2.mmmu.textown-notes.hi\endcsname{$-$0.5}
\expandafter\def\csname N@e2.mmmu.textown-notes.lo\endcsname{$-$6.8}
\expandafter\def\csname N@e2.mmmu.textown-own\endcsname{$-$3.2}
\expandafter\def\csname N@e2.mmmu.textown-own.abs\endcsname{3.2}
\expandafter\def\csname N@e2.mmmu.textown-own.ci\endcsname{[$-$6.8, 0.0]}
\expandafter\def\csname N@e2.mmmu.textown-own.hi\endcsname{0.0}
\expandafter\def\csname N@e2.mmmu.textown-own.lo\endcsname{$-$6.8}
\expandafter\def\csname N@e2.mmmu.textown-textempty\endcsname{+22.0}
\expandafter\def\csname N@e2.mmmu.textown-textempty.abs\endcsname{22.0}
\expandafter\def\csname N@e2.mmmu.textown-textempty.ci\endcsname{[+15.0, +29.0]}
\expandafter\def\csname N@e2.mmmu.textown-textempty.hi\endcsname{+29.0}
\expandafter\def\csname N@e2.mmmu.textown-textempty.lo\endcsname{+15.0}
\expandafter\def\csname N@e2.mmmu.textown.acc\endcsname{79.8}
\expandafter\def\csname N@e2.mmmu.textown.prompt\endcsname{761}
\expandafter\def\csname N@e2.mmmu.textown.t\endcsname{0.067}
\expandafter\def\csname N@e2.mmmu.textown.t.ci\endcsname{[0.051, 0.088]}
\expandafter\def\csname N@e2.mmmu.textown.t.pct\endcsname{6.7}
\expandafter\def\csname N@e2.mmmu.textown.tok\endcsname{1,887}
\expandafter\def\csname N@e2.mmmu.textshare\endcsname{87}
\expandafter\def\csname N@e2.vh.blind-textempty\endcsname{+18.5}
\expandafter\def\csname N@e2.vh.blind-textempty.abs\endcsname{18.5}
\expandafter\def\csname N@e2.vh.blind-textempty.ci\endcsname{[+14.8, +22.0]}
\expandafter\def\csname N@e2.vh.blind-textempty.hi\endcsname{+22.0}
\expandafter\def\csname N@e2.vh.blind-textempty.lo\endcsname{+14.8}
\expandafter\def\csname N@e2.vh.own.acc\endcsname{70.6}
\expandafter\def\csname N@e2.vh.own.prompt\endcsname{43,467}
\expandafter\def\csname N@e2.vh.own.t\endcsname{0.12}
\expandafter\def\csname N@e2.vh.own.t.ci\endcsname{[0.11, 0.13]}
\expandafter\def\csname N@e2.vh.own.t.pct\endcsname{12.1}
\expandafter\def\csname N@e2.vh.own.tok\endcsname{1,231}
\expandafter\def\csname N@e2.vh.reading\endcsname{video-conditioned channels carry part of it}
\expandafter\def\csname N@e2.vh.textempty.acc\endcsname{46.8}
\expandafter\def\csname N@e2.vh.textempty.prompt\endcsname{638}
\expandafter\def\csname N@e2.vh.textempty.t\endcsname{0.18}
\expandafter\def\csname N@e2.vh.textempty.t.ci\endcsname{[0.16, 0.20]}
\expandafter\def\csname N@e2.vh.textempty.t.pct\endcsname{18.0}
\expandafter\def\csname N@e2.vh.textempty.tok\endcsname{3,104}
\expandafter\def\csname N@e2.vh.textown-notes\endcsname{$-$4.8}
\expandafter\def\csname N@e2.vh.textown-notes.abs\endcsname{4.8}
\expandafter\def\csname N@e2.vh.textown-notes.ci\endcsname{[$-$7.1, $-$2.3]}
\expandafter\def\csname N@e2.vh.textown-notes.hi\endcsname{$-$2.3}
\expandafter\def\csname N@e2.vh.textown-notes.lo\endcsname{$-$7.1}
\expandafter\def\csname N@e2.vh.textown-own\endcsname{$-$4.5}
\expandafter\def\csname N@e2.vh.textown-own.abs\endcsname{4.5}
\expandafter\def\csname N@e2.vh.textown-own.ci\endcsname{[$-$6.4, $-$2.5]}
\expandafter\def\csname N@e2.vh.textown-own.hi\endcsname{$-$2.5}
\expandafter\def\csname N@e2.vh.textown-own.lo\endcsname{$-$6.4}
\expandafter\def\csname N@e2.vh.textown-textempty\endcsname{+19.3}
\expandafter\def\csname N@e2.vh.textown-textempty.abs\endcsname{19.3}
\expandafter\def\csname N@e2.vh.textown-textempty.ci\endcsname{[+15.5, +23.0]}
\expandafter\def\csname N@e2.vh.textown-textempty.hi\endcsname{+23.0}
\expandafter\def\csname N@e2.vh.textown-textempty.lo\endcsname{+15.5}
\expandafter\def\csname N@e2.vh.textown.acc\endcsname{66.1}
\expandafter\def\csname N@e2.vh.textown.prompt\endcsname{638}
\expandafter\def\csname N@e2.vh.textown.t\endcsname{0.082}
\expandafter\def\csname N@e2.vh.textown.t.ci\endcsname{[0.072, 0.093]}
\expandafter\def\csname N@e2.vh.textown.t.pct\endcsname{8.2}
\expandafter\def\csname N@e2.vh.textown.tok\endcsname{1,547}
\expandafter\def\csname N@e2.vh.textshare\endcsname{81}
\expandafter\def\csname N@e45.mmmu.RLpins-RLnotes\endcsname{+2.2}
\expandafter\def\csname N@e45.mmmu.RLpins-RLnotes.abs\endcsname{2.2}
\expandafter\def\csname N@e45.mmmu.RLpins-RLnotes.ci\endcsname{[$-$0.2, +4.8]}
\expandafter\def\csname N@e45.mmmu.RLpins-RLnotes.hi\endcsname{+4.8}
\expandafter\def\csname N@e45.mmmu.RLpins-RLnotes.lo\endcsname{$-$0.2}
\expandafter\def\csname N@e45.mmmu.blind.acc\endcsname{69.0}
\expandafter\def\csname N@e45.mmmu.blind.chars\endcsname{0}
\expandafter\def\csname N@e45.mmmu.blind.hidden\endcsname{28}
\expandafter\def\csname N@e45.mmmu.blind.t\endcsname{0.18}
\expandafter\def\csname N@e45.mmmu.blind.t.ci\endcsname{[0.14, 0.23]}
\expandafter\def\csname N@e45.mmmu.blind.t.pct\endcsname{17.9}
\expandafter\def\csname N@e45.mmmu.blind.tok\endcsname{4,073}
\expandafter\def\csname N@e45.mmmu.notes.acc\endcsname{83.2}
\expandafter\def\csname N@e45.mmmu.notes.chars\endcsname{430}
\expandafter\def\csname N@e45.mmmu.notes.hidden\endcsname{169}
\expandafter\def\csname N@e45.mmmu.notes.t\endcsname{0.13}
\expandafter\def\csname N@e45.mmmu.notes.t.ci\endcsname{[0.12, 0.16]}
\expandafter\def\csname N@e45.mmmu.notes.t.pct\endcsname{13.3}
\expandafter\def\csname N@e45.mmmu.notes.tok\endcsname{2,025}
\expandafter\def\csname N@e45.mmmu.own-blind\endcsname{+14.0}
\expandafter\def\csname N@e45.mmmu.own-blind.abs\endcsname{14.0}
\expandafter\def\csname N@e45.mmmu.own-blind.ci\endcsname{[+8.8, +19.2]}
\expandafter\def\csname N@e45.mmmu.own-blind.hi\endcsname{+19.2}
\expandafter\def\csname N@e45.mmmu.own-blind.lo\endcsname{+8.8}
\expandafter\def\csname N@e45.mmmu.own-notes\endcsname{$-$0.3}
\expandafter\def\csname N@e45.mmmu.own-notes.abs\endcsname{0.3}
\expandafter\def\csname N@e45.mmmu.own-notes.ci\endcsname{[$-$3.2, +2.5]}
\expandafter\def\csname N@e45.mmmu.own-notes.hi\endcsname{+2.5}
\expandafter\def\csname N@e45.mmmu.own-notes.lo\endcsname{$-$3.2}
\expandafter\def\csname N@e45.mmmu.own-shuffle\endcsname{$-$1.5}
\expandafter\def\csname N@e45.mmmu.own-shuffle.abs\endcsname{1.5}
\expandafter\def\csname N@e45.mmmu.own-shuffle.ci\endcsname{[$-$4.2, +1.0]}
\expandafter\def\csname N@e45.mmmu.own-shuffle.hi\endcsname{+1.0}
\expandafter\def\csname N@e45.mmmu.own-shuffle.lo\endcsname{$-$4.2}
\expandafter\def\csname N@e45.mmmu.own-swap\endcsname{+22.2}
\expandafter\def\csname N@e45.mmmu.own-swap.abs\endcsname{22.2}
\expandafter\def\csname N@e45.mmmu.own-swap.ci\endcsname{[+17.0, +27.5]}
\expandafter\def\csname N@e45.mmmu.own-swap.hi\endcsname{+27.5}
\expandafter\def\csname N@e45.mmmu.own-swap.lo\endcsname{+17.0}
\expandafter\def\csname N@e45.mmmu.own.acc\endcsname{83.0}
\expandafter\def\csname N@e45.mmmu.own.chars\endcsname{418}
\expandafter\def\csname N@e45.mmmu.own.hidden\endcsname{168}
\expandafter\def\csname N@e45.mmmu.own.t\endcsname{0.13}
\expandafter\def\csname N@e45.mmmu.own.t.ci\endcsname{[0.11, 0.14]}
\expandafter\def\csname N@e45.mmmu.own.t.pct\endcsname{12.5}
\expandafter\def\csname N@e45.mmmu.own.tok\endcsname{2,043}
\expandafter\def\csname N@e45.mmmu.rlnotes.acc\endcsname{84.2}
\expandafter\def\csname N@e45.mmmu.rlnotes.chars\endcsname{106}
\expandafter\def\csname N@e45.mmmu.rlnotes.hidden\endcsname{68}
\expandafter\def\csname N@e45.mmmu.rlnotes.t\endcsname{0.041}
\expandafter\def\csname N@e45.mmmu.rlnotes.t.ci\endcsname{[0.035, 0.049]}
\expandafter\def\csname N@e45.mmmu.rlnotes.t.pct\endcsname{4.1}
\expandafter\def\csname N@e45.mmmu.rlnotes.tok\endcsname{758}
\expandafter\def\csname N@e45.mmmu.rlpins.acc\endcsname{86.5}
\expandafter\def\csname N@e45.mmmu.rlpins.chars\endcsname{132}
\expandafter\def\csname N@e45.mmmu.rlpins.hidden\endcsname{87}
\expandafter\def\csname N@e45.mmmu.rlpins.t\endcsname{0.062}
\expandafter\def\csname N@e45.mmmu.rlpins.t.ci\endcsname{[0.051, 0.076]}
\expandafter\def\csname N@e45.mmmu.rlpins.t.pct\endcsname{6.2}
\expandafter\def\csname N@e45.mmmu.rlpins.tok\endcsname{874}
\expandafter\def\csname N@e45.mmmu.rlpins.tratio\endcsname{1.5}
\expandafter\def\csname N@e45.mmmu.shuffle.acc\endcsname{84.5}
\expandafter\def\csname N@e45.mmmu.shuffle.chars\endcsname{418}
\expandafter\def\csname N@e45.mmmu.shuffle.hidden\endcsname{168}
\expandafter\def\csname N@e45.mmmu.shuffle.t\endcsname{0.11}
\expandafter\def\csname N@e45.mmmu.shuffle.t.ci\endcsname{[0.10, 0.13]}
\expandafter\def\csname N@e45.mmmu.shuffle.t.pct\endcsname{11.2}
\expandafter\def\csname N@e45.mmmu.shuffle.tok\endcsname{1,850}
\expandafter\def\csname N@e45.mmmu.swap-blind\endcsname{$-$8.2}
\expandafter\def\csname N@e45.mmmu.swap-blind.abs\endcsname{8.2}
\expandafter\def\csname N@e45.mmmu.swap-blind.ci\endcsname{[$-$12.7, $-$3.7]}
\expandafter\def\csname N@e45.mmmu.swap-blind.hi\endcsname{$-$3.7}
\expandafter\def\csname N@e45.mmmu.swap-blind.lo\endcsname{$-$12.7}
\expandafter\def\csname N@e45.mmmu.swap.acc\endcsname{60.8}
\expandafter\def\csname N@e45.mmmu.swap.chars\endcsname{418}
\expandafter\def\csname N@e45.mmmu.swap.hidden\endcsname{168}
\expandafter\def\csname N@e45.mmmu.swap.t\endcsname{0.23}
\expandafter\def\csname N@e45.mmmu.swap.t.ci\endcsname{[0.18, 0.29]}
\expandafter\def\csname N@e45.mmmu.swap.t.pct\endcsname{22.9}
\expandafter\def\csname N@e45.mmmu.swap.tok\endcsname{4,701}
\expandafter\def\csname N@e45.mmmu.vanilla.acc\endcsname{85.8}
\expandafter\def\csname N@e45.mmmu.vanilla.tok\endcsname{3,425}
\expandafter\def\csname N@e45.vh.RLpins-RLnotes\endcsname{+0.9}
\expandafter\def\csname N@e45.vh.RLpins-RLnotes.abs\endcsname{0.9}
\expandafter\def\csname N@e45.vh.RLpins-RLnotes.ci\endcsname{[$-$0.5, +2.4]}
\expandafter\def\csname N@e45.vh.RLpins-RLnotes.hi\endcsname{+2.4}
\expandafter\def\csname N@e45.vh.RLpins-RLnotes.lo\endcsname{$-$0.5}
\expandafter\def\csname N@e45.vh.blind.acc\endcsname{65.3}
\expandafter\def\csname N@e45.vh.blind.chars\endcsname{0}
\expandafter\def\csname N@e45.vh.blind.hidden\endcsname{28}
\expandafter\def\csname N@e45.vh.blind.t\endcsname{0.13}
\expandafter\def\csname N@e45.vh.blind.t.ci\endcsname{[0.11, 0.16]}
\expandafter\def\csname N@e45.vh.blind.t.pct\endcsname{13.3}
\expandafter\def\csname N@e45.vh.blind.tok\endcsname{1,858}
\expandafter\def\csname N@e45.vh.notes.acc\endcsname{70.9}
\expandafter\def\csname N@e45.vh.notes.chars\endcsname{566}
\expandafter\def\csname N@e45.vh.notes.hidden\endcsname{200}
\expandafter\def\csname N@e45.vh.notes.t\endcsname{0.12}
\expandafter\def\csname N@e45.vh.notes.t.ci\endcsname{[0.11, 0.13]}
\expandafter\def\csname N@e45.vh.notes.t.pct\endcsname{11.8}
\expandafter\def\csname N@e45.vh.notes.tok\endcsname{1,199}
\expandafter\def\csname N@e45.vh.own-blind\endcsname{+5.3}
\expandafter\def\csname N@e45.vh.own-blind.abs\endcsname{5.3}
\expandafter\def\csname N@e45.vh.own-blind.ci\endcsname{[+2.6, +8.1]}
\expandafter\def\csname N@e45.vh.own-blind.hi\endcsname{+8.1}
\expandafter\def\csname N@e45.vh.own-blind.lo\endcsname{+2.6}
\expandafter\def\csname N@e45.vh.own-notes\endcsname{$-$0.3}
\expandafter\def\csname N@e45.vh.own-notes.abs\endcsname{0.3}
\expandafter\def\csname N@e45.vh.own-notes.ci\endcsname{[$-$2.3, +1.6]}
\expandafter\def\csname N@e45.vh.own-notes.hi\endcsname{+1.6}
\expandafter\def\csname N@e45.vh.own-notes.lo\endcsname{$-$2.3}
\expandafter\def\csname N@e45.vh.own-shuffle\endcsname{+0.2}
\expandafter\def\csname N@e45.vh.own-shuffle.abs\endcsname{0.2}
\expandafter\def\csname N@e45.vh.own-shuffle.ci\endcsname{[$-$1.6, +1.9]}
\expandafter\def\csname N@e45.vh.own-shuffle.hi\endcsname{+1.9}
\expandafter\def\csname N@e45.vh.own-shuffle.lo\endcsname{$-$1.6}
\expandafter\def\csname N@e45.vh.own-swap\endcsname{+17.0}
\expandafter\def\csname N@e45.vh.own-swap.abs\endcsname{17.0}
\expandafter\def\csname N@e45.vh.own-swap.ci\endcsname{[+13.3, +20.7]}
\expandafter\def\csname N@e45.vh.own-swap.hi\endcsname{+20.7}
\expandafter\def\csname N@e45.vh.own-swap.lo\endcsname{+13.3}
\expandafter\def\csname N@e45.vh.own.acc\endcsname{70.6}
\expandafter\def\csname N@e45.vh.own.chars\endcsname{568}
\expandafter\def\csname N@e45.vh.own.hidden\endcsname{200}
\expandafter\def\csname N@e45.vh.own.t\endcsname{0.12}
\expandafter\def\csname N@e45.vh.own.t.ci\endcsname{[0.11, 0.13]}
\expandafter\def\csname N@e45.vh.own.t.pct\endcsname{12.1}
\expandafter\def\csname N@e45.vh.own.tok\endcsname{1,231}
\expandafter\def\csname N@e45.vh.rlnotes.acc\endcsname{74.3}
\expandafter\def\csname N@e45.vh.rlnotes.chars\endcsname{155}
\expandafter\def\csname N@e45.vh.rlnotes.hidden\endcsname{66}
\expandafter\def\csname N@e45.vh.rlnotes.t\endcsname{0.041}
\expandafter\def\csname N@e45.vh.rlnotes.t.ci\endcsname{[0.038, 0.043]}
\expandafter\def\csname N@e45.vh.rlnotes.t.pct\endcsname{4.1}
\expandafter\def\csname N@e45.vh.rlnotes.tok\endcsname{505}
\expandafter\def\csname N@e45.vh.rlpins.acc\endcsname{75.2}
\expandafter\def\csname N@e45.vh.rlpins.chars\endcsname{189}
\expandafter\def\csname N@e45.vh.rlpins.hidden\endcsname{93}
\expandafter\def\csname N@e45.vh.rlpins.t\endcsname{0.069}
\expandafter\def\csname N@e45.vh.rlpins.t.ci\endcsname{[0.064, 0.074]}
\expandafter\def\csname N@e45.vh.rlpins.t.pct\endcsname{6.9}
\expandafter\def\csname N@e45.vh.rlpins.tok\endcsname{633}
\expandafter\def\csname N@e45.vh.rlpins.tratio\endcsname{1.7}
\expandafter\def\csname N@e45.vh.shuffle.acc\endcsname{70.4}
\expandafter\def\csname N@e45.vh.shuffle.chars\endcsname{568}
\expandafter\def\csname N@e45.vh.shuffle.hidden\endcsname{200}
\expandafter\def\csname N@e45.vh.shuffle.t\endcsname{0.13}
\expandafter\def\csname N@e45.vh.shuffle.t.ci\endcsname{[0.12, 0.14]}
\expandafter\def\csname N@e45.vh.shuffle.t.pct\endcsname{12.6}
\expandafter\def\csname N@e45.vh.shuffle.tok\endcsname{1,308}
\expandafter\def\csname N@e45.vh.swap-blind\endcsname{$-$11.7}
\expandafter\def\csname N@e45.vh.swap-blind.abs\endcsname{11.7}
\expandafter\def\csname N@e45.vh.swap-blind.ci\endcsname{[$-$15.1, $-$8.3]}
\expandafter\def\csname N@e45.vh.swap-blind.hi\endcsname{$-$8.3}
\expandafter\def\csname N@e45.vh.swap-blind.lo\endcsname{$-$15.1}
\expandafter\def\csname N@e45.vh.swap.acc\endcsname{53.6}
\expandafter\def\csname N@e45.vh.swap.chars\endcsname{568}
\expandafter\def\csname N@e45.vh.swap.hidden\endcsname{200}
\expandafter\def\csname N@e45.vh.swap.t\endcsname{0.27}
\expandafter\def\csname N@e45.vh.swap.t.ci\endcsname{[0.24, 0.30]}
\expandafter\def\csname N@e45.vh.swap.t.pct\endcsname{26.7}
\expandafter\def\csname N@e45.vh.swap.tok\endcsname{3,460}
\expandafter\def\csname N@e45.vh.vanilla.acc\endcsname{71.3}
\expandafter\def\csname N@e45.vh.vanilla.tok\endcsname{3,162}
\expandafter\def\csname N@eff.lvb.notes.open\endcsname{1.0}
\expandafter\def\csname N@eff.lvb.nothink.acc\endcsname{66.7}
\expandafter\def\csname N@eff.lvb.ntnotes.acc\endcsname{65.7}
\expandafter\def\csname N@eff.lvb.ntnotes.d\endcsname{$-$1.0}
\expandafter\def\csname N@eff.lvb.ntnotes.d.abs\endcsname{1.0}
\expandafter\def\csname N@eff.lvb.ntnotes.d.ci\endcsname{[$-$5.7, +3.7]}
\expandafter\def\csname N@eff.lvb.ntnotes.d.hi\endcsname{+3.7}
\expandafter\def\csname N@eff.lvb.ntnotes.d.lo\endcsname{$-$5.7}
\expandafter\def\csname N@eff.lvb.ntnotes.hidden\endcsname{97}
\expandafter\def\csname N@eff.lvb.ntnotes.open\endcsname{0.3}
\expandafter\def\csname N@eff.lvb.ntnotes.t\endcsname{0.57}
\expandafter\def\csname N@eff.lvb.ntnotes.t.ci\endcsname{[0.43, 0.77]}
\expandafter\def\csname N@eff.lvb.ntnotes.t.pct\endcsname{57.1}
\expandafter\def\csname N@eff.mmmu.notes.open\endcsname{0.7}
\expandafter\def\csname N@eff.mmmu.nothink.acc\endcsname{84.2}
\expandafter\def\csname N@eff.mmmu.ntnotes.acc\endcsname{85.2}
\expandafter\def\csname N@eff.mmmu.ntnotes.d\endcsname{+1.0}
\expandafter\def\csname N@eff.mmmu.ntnotes.d.abs\endcsname{1.0}
\expandafter\def\csname N@eff.mmmu.ntnotes.d.ci\endcsname{[$-$3.0, +5.0]}
\expandafter\def\csname N@eff.mmmu.ntnotes.d.hi\endcsname{+5.0}
\expandafter\def\csname N@eff.mmmu.ntnotes.d.lo\endcsname{$-$3.0}
\expandafter\def\csname N@eff.mmmu.ntnotes.hidden\endcsname{131}
\expandafter\def\csname N@eff.mmmu.ntnotes.open\endcsname{0.2}
\expandafter\def\csname N@eff.mmmu.ntnotes.t\endcsname{0.30}
\expandafter\def\csname N@eff.mmmu.ntnotes.t.ci\endcsname{[0.27, 0.34]}
\expandafter\def\csname N@eff.mmmu.ntnotes.t.pct\endcsname{30.2}
\expandafter\def\csname N@eff.vh.notes.open\endcsname{0.0}
\expandafter\def\csname N@eff.vh.nothink.acc\endcsname{71.0}
\expandafter\def\csname N@eff.vh.ntnotes.acc\endcsname{69.6}
\expandafter\def\csname N@eff.vh.ntnotes.d\endcsname{$-$1.4}
\expandafter\def\csname N@eff.vh.ntnotes.d.abs\endcsname{1.4}
\expandafter\def\csname N@eff.vh.ntnotes.d.ci\endcsname{[$-$4.2, +1.2]}
\expandafter\def\csname N@eff.vh.ntnotes.d.hi\endcsname{+1.2}
\expandafter\def\csname N@eff.vh.ntnotes.d.lo\endcsname{$-$4.2}
\expandafter\def\csname N@eff.vh.ntnotes.hidden\endcsname{153}
\expandafter\def\csname N@eff.vh.ntnotes.open\endcsname{0.2}
\expandafter\def\csname N@eff.vh.ntnotes.t\endcsname{0.67}
\expandafter\def\csname N@eff.vh.ntnotes.t.ci\endcsname{[0.63, 0.72]}
\expandafter\def\csname N@eff.vh.ntnotes.t.pct\endcsname{67.3}
\expandafter\def\csname N@eff.vh.split.cut\endcsname{215}
\expandafter\def\csname N@eff.vh.split.long\endcsname{0.46}
\expandafter\def\csname N@eff.vh.split.short\endcsname{1.35}
\expandafter\def\csname N@gate.hit.model\endcsname{0.612}
\expandafter\def\csname N@gate.hit.siglip\endcsname{0.588}
\expandafter\def\csname N@gate.mmmu.G1\endcsname{+1.5}
\expandafter\def\csname N@gate.mmmu.G1.abs\endcsname{1.5}
\expandafter\def\csname N@gate.mmmu.G1.ci\endcsname{[$-$1.7, +4.7]}
\expandafter\def\csname N@gate.mmmu.G1.hi\endcsname{+4.7}
\expandafter\def\csname N@gate.mmmu.G1.lo\endcsname{$-$1.7}
\expandafter\def\csname N@gate.mmmu.pins-notes\endcsname{$-$0.3}
\expandafter\def\csname N@gate.mmmu.pins-notes.abs\endcsname{0.3}
\expandafter\def\csname N@gate.mmmu.pins-notes.ci\endcsname{[$-$3.0, +2.5]}
\expandafter\def\csname N@gate.mmmu.pins-notes.hi\endcsname{+2.5}
\expandafter\def\csname N@gate.mmmu.pins-notes.lo\endcsname{$-$3.0}
\expandafter\def\csname N@gate.mmmu.pins-pinsrandom\endcsname{$-$1.5}
\expandafter\def\csname N@gate.mmmu.pins-pinsrandom.abs\endcsname{1.5}
\expandafter\def\csname N@gate.mmmu.pins-pinsrandom.ci\endcsname{[$-$5.5, +2.5]}
\expandafter\def\csname N@gate.mmmu.pins-pinsrandom.hi\endcsname{+2.5}
\expandafter\def\csname N@gate.mmmu.pins-pinsrandom.lo\endcsname{$-$5.5}
\expandafter\def\csname N@gate.mmmu.pins-pinssiglip\endcsname{$-$1.0}
\expandafter\def\csname N@gate.mmmu.pins-pinssiglip.abs\endcsname{1.0}
\expandafter\def\csname N@gate.mmmu.pins-pinssiglip.ci\endcsname{[$-$4.0, +2.0]}
\expandafter\def\csname N@gate.mmmu.pins-pinssiglip.hi\endcsname{+2.0}
\expandafter\def\csname N@gate.mmmu.pins-pinssiglip.lo\endcsname{$-$4.0}
\expandafter\def\csname N@gate.mmmu.pins.acc\endcsname{83.0}
\expandafter\def\csname N@gate.mmmu.pinsrandom.acc\endcsname{83.5}
\expandafter\def\csname N@gate.mmmu.pinssiglip.acc\endcsname{83.0}
\expandafter\def\csname N@gate.mmmu.vanilla-notes\endcsname{+2.5}
\expandafter\def\csname N@gate.mmmu.vanilla-notes.abs\endcsname{2.5}
\expandafter\def\csname N@gate.mmmu.vanilla-notes.ci\endcsname{[$-$0.2, +5.2]}
\expandafter\def\csname N@gate.mmmu.vanilla-notes.hi\endcsname{+5.2}
\expandafter\def\csname N@gate.mmmu.vanilla-notes.lo\endcsname{$-$0.2}
\expandafter\def\csname N@gate.vh.G1\endcsname{+0.3}
\expandafter\def\csname N@gate.vh.G1.abs\endcsname{0.3}
\expandafter\def\csname N@gate.vh.G1.ci\endcsname{[$-$2.3, +2.9]}
\expandafter\def\csname N@gate.vh.G1.hi\endcsname{+2.9}
\expandafter\def\csname N@gate.vh.G1.lo\endcsname{$-$2.3}
\expandafter\def\csname N@gate.vh.pins-notes\endcsname{$-$1.7}
\expandafter\def\csname N@gate.vh.pins-notes.abs\endcsname{1.7}
\expandafter\def\csname N@gate.vh.pins-notes.ci\endcsname{[$-$4.0, +0.5]}
\expandafter\def\csname N@gate.vh.pins-notes.hi\endcsname{+0.5}
\expandafter\def\csname N@gate.vh.pins-notes.lo\endcsname{$-$4.0}
\expandafter\def\csname N@gate.vh.pins-pinsrandom\endcsname{$-$1.5}
\expandafter\def\csname N@gate.vh.pins-pinsrandom.abs\endcsname{1.5}
\expandafter\def\csname N@gate.vh.pins-pinsrandom.ci\endcsname{[$-$4.6, +1.4]}
\expandafter\def\csname N@gate.vh.pins-pinsrandom.hi\endcsname{+1.4}
\expandafter\def\csname N@gate.vh.pins-pinsrandom.lo\endcsname{$-$4.6}
\expandafter\def\csname N@gate.vh.pins-pinssiglip\endcsname{$-$0.5}
\expandafter\def\csname N@gate.vh.pins-pinssiglip.abs\endcsname{0.5}
\expandafter\def\csname N@gate.vh.pins-pinssiglip.ci\endcsname{[$-$3.0, +2.1]}
\expandafter\def\csname N@gate.vh.pins-pinssiglip.hi\endcsname{+2.1}
\expandafter\def\csname N@gate.vh.pins-pinssiglip.lo\endcsname{$-$3.0}
\expandafter\def\csname N@gate.vh.pins.acc\endcsname{69.1}
\expandafter\def\csname N@gate.vh.pinsrandom.acc\endcsname{70.8}
\expandafter\def\csname N@gate.vh.pinssiglip.acc\endcsname{69.7}
\expandafter\def\csname N@gate.vh.vanilla-notes\endcsname{+0.5}
\expandafter\def\csname N@gate.vh.vanilla-notes.abs\endcsname{0.5}
\expandafter\def\csname N@gate.vh.vanilla-notes.ci\endcsname{[$-$1.8, +2.8]}
\expandafter\def\csname N@gate.vh.vanilla-notes.hi\endcsname{+2.8}
\expandafter\def\csname N@gate.vh.vanilla-notes.lo\endcsname{$-$1.8}
\expandafter\def\csname N@in.lvb.cmp.nothink.f192-rlnotes.d\endcsname{$-$9.5}
\expandafter\def\csname N@in.lvb.cmp.nothink.f192-rlnotes.d.abs\endcsname{9.5}
\expandafter\def\csname N@in.lvb.cmp.nothink.f192-rlnotes.d.ci\endcsname{[$-$12.2, $-$6.8]}
\expandafter\def\csname N@in.lvb.cmp.nothink.f192-rlnotes.d.hi\endcsname{$-$6.8}
\expandafter\def\csname N@in.lvb.cmp.nothink.f192-rlnotes.d.lo\endcsname{$-$12.2}
\expandafter\def\csname N@in.lvb.cmp.nothink.f192-rlnotes.match\endcsname{no}
\expandafter\def\csname N@in.lvb.cmp.nothink.f192-rlnotes.t\endcsname{1.31}
\expandafter\def\csname N@in.lvb.cmp.nothink.f192-rlnotes.t.ci\endcsname{[1.18, 1.43]}
\expandafter\def\csname N@in.lvb.cmp.nothink.f192-rlnotes.t.pct\endcsname{130.8}
\expandafter\def\csname N@in.lvb.cmp.nothink.vc2-rlnotes.d\endcsname{$-$2.4}
\expandafter\def\csname N@in.lvb.cmp.nothink.vc2-rlnotes.d.abs\endcsname{2.4}
\expandafter\def\csname N@in.lvb.cmp.nothink.vc2-rlnotes.d.ci\endcsname{[$-$4.8, 0.0]}
\expandafter\def\csname N@in.lvb.cmp.nothink.vc2-rlnotes.d.hi\endcsname{0.0}
\expandafter\def\csname N@in.lvb.cmp.nothink.vc2-rlnotes.d.lo\endcsname{$-$4.8}
\expandafter\def\csname N@in.lvb.cmp.nothink.vc2-rlnotes.match\endcsname{no}
\expandafter\def\csname N@in.lvb.cmp.nothink.vc2-rlnotes.t\endcsname{1.05}
\expandafter\def\csname N@in.lvb.cmp.nothink.vc2-rlnotes.t.ci\endcsname{[0.91, 1.20]}
\expandafter\def\csname N@in.lvb.cmp.nothink.vc2-rlnotes.t.pct\endcsname{105.2}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.f192-rlvan.f192.d\endcsname{$-$1.4}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.f192-rlvan.f192.d.abs\endcsname{1.4}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.f192-rlvan.f192.d.ci\endcsname{[$-$3.6, +0.9]}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.f192-rlvan.f192.d.hi\endcsname{+0.9}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.f192-rlvan.f192.d.lo\endcsname{$-$3.6}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.f192-rlvan.f192.t\endcsname{0.71}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.f192-rlvan.f192.t.ci\endcsname{[0.69, 0.72]}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.f192-rlvan.f192.t.pct\endcsname{70.5}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.vc2-rlvan.vc2.d\endcsname{$-$1.6}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.vc2-rlvan.vc2.d.abs\endcsname{1.6}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.vc2-rlvan.vc2.d.ci\endcsname{[$-$3.7, +0.4]}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.vc2-rlvan.vc2.d.hi\endcsname{+0.4}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.vc2-rlvan.vc2.d.lo\endcsname{$-$3.7}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.vc2-rlvan.vc2.t\endcsname{0.66}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.vc2-rlvan.vc2.t.ci\endcsname{[0.64, 0.70]}
\expandafter\def\csname N@in.lvb.cmp.rlnotes.vc2-rlvan.vc2.t.pct\endcsname{66.2}
\expandafter\def\csname N@in.lvb.cmp.rlvan.f192-rlnotes.d\endcsname{$-$8.8}
\expandafter\def\csname N@in.lvb.cmp.rlvan.f192-rlnotes.d.abs\endcsname{8.8}
\expandafter\def\csname N@in.lvb.cmp.rlvan.f192-rlnotes.d.ci\endcsname{[$-$11.5, $-$6.0]}
\expandafter\def\csname N@in.lvb.cmp.rlvan.f192-rlnotes.d.hi\endcsname{$-$6.0}
\expandafter\def\csname N@in.lvb.cmp.rlvan.f192-rlnotes.d.lo\endcsname{$-$11.5}
\expandafter\def\csname N@in.lvb.cmp.rlvan.f192-rlnotes.match\endcsname{no}
\expandafter\def\csname N@in.lvb.cmp.rlvan.f192-rlnotes.t\endcsname{0.67}
\expandafter\def\csname N@in.lvb.cmp.rlvan.f192-rlnotes.t.ci\endcsname{[0.66, 0.69]}
\expandafter\def\csname N@in.lvb.cmp.rlvan.f192-rlnotes.t.pct\endcsname{67.4}
\expandafter\def\csname N@in.lvb.cmp.rlvan.vc2-rlnotes.d\endcsname{$-$1.8}
\expandafter\def\csname N@in.lvb.cmp.rlvan.vc2-rlnotes.d.abs\endcsname{1.8}
\expandafter\def\csname N@in.lvb.cmp.rlvan.vc2-rlnotes.d.ci\endcsname{[$-$4.1, +0.3]}
\expandafter\def\csname N@in.lvb.cmp.rlvan.vc2-rlnotes.d.hi\endcsname{+0.3}
\expandafter\def\csname N@in.lvb.cmp.rlvan.vc2-rlnotes.d.lo\endcsname{$-$4.1}
\expandafter\def\csname N@in.lvb.cmp.rlvan.vc2-rlnotes.match\endcsname{no}
\expandafter\def\csname N@in.lvb.cmp.rlvan.vc2-rlnotes.t\endcsname{0.78}
\expandafter\def\csname N@in.lvb.cmp.rlvan.vc2-rlnotes.t.ci\endcsname{[0.76, 0.80]}
\expandafter\def\csname N@in.lvb.cmp.rlvan.vc2-rlnotes.t.pct\endcsname{77.9}
\expandafter\def\csname N@in.lvb.nnerr\endcsname{5.4}
\expandafter\def\csname N@in.lvb.nothink.f192.acc\endcsname{54.2}
\expandafter\def\csname N@in.lvb.nothink.f192.d\endcsname{$-$12.3}
\expandafter\def\csname N@in.lvb.nothink.f192.d.abs\endcsname{12.3}
\expandafter\def\csname N@in.lvb.nothink.f192.d.ci\endcsname{[$-$15.5, $-$9.2]}
\expandafter\def\csname N@in.lvb.nothink.f192.d.hi\endcsname{$-$9.2}
\expandafter\def\csname N@in.lvb.nothink.f192.d.lo\endcsname{$-$15.5}
\expandafter\def\csname N@in.lvb.nothink.f192.own\endcsname{$-$12.1}
\expandafter\def\csname N@in.lvb.nothink.f192.own.abs\endcsname{12.1}
\expandafter\def\csname N@in.lvb.nothink.f192.own.ci\endcsname{[$-$15.0, $-$9.1]}
\expandafter\def\csname N@in.lvb.nothink.f192.own.hi\endcsname{$-$9.1}
\expandafter\def\csname N@in.lvb.nothink.f192.own.lo\endcsname{$-$15.0}
\expandafter\def\csname N@in.lvb.nothink.f192.prompt\endcsname{22,107}
\expandafter\def\csname N@in.lvb.nothink.f192.promptk\endcsname{22.1K}
\expandafter\def\csname N@in.lvb.nothink.f192.t\endcsname{0.030}
\expandafter\def\csname N@in.lvb.nothink.f192.t.ci\endcsname{[0.026, 0.034]}
\expandafter\def\csname N@in.lvb.nothink.f192.t.pct\endcsname{3.0}
\expandafter\def\csname N@in.lvb.nothink.f192.tok\endcsname{296}
\expandafter\def\csname N@in.lvb.nothink.f192.vsown.t\endcsname{0.50}
\expandafter\def\csname N@in.lvb.nothink.vc2.acc\endcsname{61.3}
\expandafter\def\csname N@in.lvb.nothink.vc2.d\endcsname{$-$5.2}
\expandafter\def\csname N@in.lvb.nothink.vc2.d.abs\endcsname{5.2}
\expandafter\def\csname N@in.lvb.nothink.vc2.d.ci\endcsname{[$-$7.5, $-$2.9]}
\expandafter\def\csname N@in.lvb.nothink.vc2.d.hi\endcsname{$-$2.9}
\expandafter\def\csname N@in.lvb.nothink.vc2.d.lo\endcsname{$-$7.5}
\expandafter\def\csname N@in.lvb.nothink.vc2.own\endcsname{$-$4.9}
\expandafter\def\csname N@in.lvb.nothink.vc2.own.abs\endcsname{4.9}
\expandafter\def\csname N@in.lvb.nothink.vc2.own.ci\endcsname{[$-$6.7, $-$3.2]}
\expandafter\def\csname N@in.lvb.nothink.vc2.own.hi\endcsname{$-$3.2}
\expandafter\def\csname N@in.lvb.nothink.vc2.own.lo\endcsname{$-$6.7}
\expandafter\def\csname N@in.lvb.nothink.vc2.prompt\endcsname{25,962}
\expandafter\def\csname N@in.lvb.nothink.vc2.promptk\endcsname{26.0K}
\expandafter\def\csname N@in.lvb.nothink.vc2.t\endcsname{0.024}
\expandafter\def\csname N@in.lvb.nothink.vc2.t.ci\endcsname{[0.021, 0.027]}
\expandafter\def\csname N@in.lvb.nothink.vc2.t.pct\endcsname{2.4}
\expandafter\def\csname N@in.lvb.nothink.vc2.tok\endcsname{209}
\expandafter\def\csname N@in.lvb.nothink.vc2.vsown.t\endcsname{0.40}
\expandafter\def\csname N@in.lvb.rlnotes.f192.acc\endcsname{53.6}
\expandafter\def\csname N@in.lvb.rlnotes.f192.d\endcsname{$-$13.0}
\expandafter\def\csname N@in.lvb.rlnotes.f192.d.abs\endcsname{13.0}
\expandafter\def\csname N@in.lvb.rlnotes.f192.d.ci\endcsname{[$-$16.3, $-$9.7]}
\expandafter\def\csname N@in.lvb.rlnotes.f192.d.hi\endcsname{$-$9.7}
\expandafter\def\csname N@in.lvb.rlnotes.f192.d.lo\endcsname{$-$16.3}
\expandafter\def\csname N@in.lvb.rlnotes.f192.own\endcsname{$-$10.1}
\expandafter\def\csname N@in.lvb.rlnotes.f192.own.abs\endcsname{10.1}
\expandafter\def\csname N@in.lvb.rlnotes.f192.own.ci\endcsname{[$-$12.8, $-$7.6]}
\expandafter\def\csname N@in.lvb.rlnotes.f192.own.hi\endcsname{$-$7.6}
\expandafter\def\csname N@in.lvb.rlnotes.f192.own.lo\endcsname{$-$12.8}
\expandafter\def\csname N@in.lvb.rlnotes.f192.prompt\endcsname{22,556}
\expandafter\def\csname N@in.lvb.rlnotes.f192.promptk\endcsname{22.6K}
\expandafter\def\csname N@in.lvb.rlnotes.f192.t\endcsname{0.011}
\expandafter\def\csname N@in.lvb.rlnotes.f192.t.ci\endcsname{[0.010, 0.012]}
\expandafter\def\csname N@in.lvb.rlnotes.f192.t.pct\endcsname{1.1}
\expandafter\def\csname N@in.lvb.rlnotes.f192.tok\endcsname{273}
\expandafter\def\csname N@in.lvb.rlnotes.f192.vsown.t\endcsname{0.48}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.acc\endcsname{60.2}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.d\endcsname{$-$6.3}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.d.abs\endcsname{6.3}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.d.ci\endcsname{[$-$8.4, $-$4.2]}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.d.hi\endcsname{$-$4.2}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.d.lo\endcsname{$-$8.4}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.own\endcsname{$-$3.5}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.own.abs\endcsname{3.5}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.own.ci\endcsname{[$-$5.3, $-$1.7]}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.own.hi\endcsname{$-$1.7}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.own.lo\endcsname{$-$5.3}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.prompt\endcsname{26,411}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.promptk\endcsname{26.4K}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.t\endcsname{0.012}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.t.ci\endcsname{[0.010, 0.013]}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.t.pct\endcsname{1.2}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.tok\endcsname{279}
\expandafter\def\csname N@in.lvb.rlnotes.vc2.vsown.t\endcsname{0.52}
\expandafter\def\csname N@in.lvb.rlvan.f192.acc\endcsname{54.9}
\expandafter\def\csname N@in.lvb.rlvan.f192.d\endcsname{$-$11.6}
\expandafter\def\csname N@in.lvb.rlvan.f192.d.abs\endcsname{11.6}
\expandafter\def\csname N@in.lvb.rlvan.f192.d.ci\endcsname{[$-$14.9, $-$8.4]}
\expandafter\def\csname N@in.lvb.rlvan.f192.d.hi\endcsname{$-$8.4}
\expandafter\def\csname N@in.lvb.rlvan.f192.d.lo\endcsname{$-$14.9}
\expandafter\def\csname N@in.lvb.rlvan.f192.own\endcsname{$-$8.7}
\expandafter\def\csname N@in.lvb.rlvan.f192.own.abs\endcsname{8.7}
\expandafter\def\csname N@in.lvb.rlvan.f192.own.ci\endcsname{[$-$11.4, $-$6.0]}
\expandafter\def\csname N@in.lvb.rlvan.f192.own.hi\endcsname{$-$6.0}
\expandafter\def\csname N@in.lvb.rlvan.f192.own.lo\endcsname{$-$11.4}
\expandafter\def\csname N@in.lvb.rlvan.f192.prompt\endcsname{22,105}
\expandafter\def\csname N@in.lvb.rlvan.f192.promptk\endcsname{22.1K}
\expandafter\def\csname N@in.lvb.rlvan.f192.t\endcsname{0.015}
\expandafter\def\csname N@in.lvb.rlvan.f192.t.ci\endcsname{[0.014, 0.017]}
\expandafter\def\csname N@in.lvb.rlvan.f192.t.pct\endcsname{1.5}
\expandafter\def\csname N@in.lvb.rlvan.f192.tok\endcsname{154}
\expandafter\def\csname N@in.lvb.rlvan.f192.vsown.t\endcsname{0.29}
\expandafter\def\csname N@in.lvb.rlvan.vc2.acc\endcsname{61.9}
\expandafter\def\csname N@in.lvb.rlvan.vc2.d\endcsname{$-$4.7}
\expandafter\def\csname N@in.lvb.rlvan.vc2.d.abs\endcsname{4.7}
\expandafter\def\csname N@in.lvb.rlvan.vc2.d.ci\endcsname{[$-$7.1, $-$2.3]}
\expandafter\def\csname N@in.lvb.rlvan.vc2.d.hi\endcsname{$-$2.3}
\expandafter\def\csname N@in.lvb.rlvan.vc2.d.lo\endcsname{$-$7.1}
\expandafter\def\csname N@in.lvb.rlvan.vc2.own\endcsname{$-$1.7}
\expandafter\def\csname N@in.lvb.rlvan.vc2.own.abs\endcsname{1.7}
\expandafter\def\csname N@in.lvb.rlvan.vc2.own.ci\endcsname{[$-$3.6, +0.1]}
\expandafter\def\csname N@in.lvb.rlvan.vc2.own.hi\endcsname{+0.1}
\expandafter\def\csname N@in.lvb.rlvan.vc2.own.lo\endcsname{$-$3.6}
\expandafter\def\csname N@in.lvb.rlvan.vc2.prompt\endcsname{25,960}
\expandafter\def\csname N@in.lvb.rlvan.vc2.promptk\endcsname{26.0K}
\expandafter\def\csname N@in.lvb.rlvan.vc2.t\endcsname{0.018}
\expandafter\def\csname N@in.lvb.rlvan.vc2.t.ci\endcsname{[0.016, 0.020]}
\expandafter\def\csname N@in.lvb.rlvan.vc2.t.pct\endcsname{1.8}
\expandafter\def\csname N@in.lvb.rlvan.vc2.tok\endcsname{157}
\expandafter\def\csname N@in.lvb.rlvan.vc2.vsown.t\endcsname{0.34}
\expandafter\def\csname N@in.mmmu.cmp.nothink.f192-rlnotes.d\endcsname{+1.0}
\expandafter\def\csname N@in.mmmu.cmp.nothink.f192-rlnotes.d.abs\endcsname{1.0}
\expandafter\def\csname N@in.mmmu.cmp.nothink.f192-rlnotes.d.ci\endcsname{[$-$1.1, +3.1]}
\expandafter\def\csname N@in.mmmu.cmp.nothink.f192-rlnotes.d.hi\endcsname{+3.1}
\expandafter\def\csname N@in.mmmu.cmp.nothink.f192-rlnotes.d.lo\endcsname{$-$1.1}
\expandafter\def\csname N@in.mmmu.cmp.nothink.f192-rlnotes.match\endcsname{no}
\expandafter\def\csname N@in.mmmu.cmp.nothink.f192-rlnotes.t\endcsname{1.47}
\expandafter\def\csname N@in.mmmu.cmp.nothink.f192-rlnotes.t.ci\endcsname{[1.24, 1.76]}
\expandafter\def\csname N@in.mmmu.cmp.nothink.f192-rlnotes.t.pct\endcsname{147.2}
\expandafter\def\csname N@in.mmmu.cmp.nothink.vc2-rlnotes.d\endcsname{$-$8.5}
\expandafter\def\csname N@in.mmmu.cmp.nothink.vc2-rlnotes.d.abs\endcsname{8.5}
\expandafter\def\csname N@in.mmmu.cmp.nothink.vc2-rlnotes.d.ci\endcsname{[$-$11.8, $-$5.2]}
\expandafter\def\csname N@in.mmmu.cmp.nothink.vc2-rlnotes.d.hi\endcsname{$-$5.2}
\expandafter\def\csname N@in.mmmu.cmp.nothink.vc2-rlnotes.d.lo\endcsname{$-$11.8}
\expandafter\def\csname N@in.mmmu.cmp.nothink.vc2-rlnotes.match\endcsname{no}
\expandafter\def\csname N@in.mmmu.cmp.nothink.vc2-rlnotes.t\endcsname{2.00}
\expandafter\def\csname N@in.mmmu.cmp.nothink.vc2-rlnotes.t.ci\endcsname{[1.63, 2.45]}
\expandafter\def\csname N@in.mmmu.cmp.nothink.vc2-rlnotes.t.pct\endcsname{200.4}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.f192-rlvan.f192.d\endcsname{+0.5}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.f192-rlvan.f192.d.abs\endcsname{0.5}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.f192-rlvan.f192.d.ci\endcsname{[$-$1.6, +2.6]}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.f192-rlvan.f192.d.hi\endcsname{+2.6}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.f192-rlvan.f192.d.lo\endcsname{$-$1.6}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.f192-rlvan.f192.t\endcsname{0.75}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.f192-rlvan.f192.t.ci\endcsname{[0.64, 0.88]}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.f192-rlvan.f192.t.pct\endcsname{74.9}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.vc2-rlvan.vc2.d\endcsname{$-$1.4}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.vc2-rlvan.vc2.d.abs\endcsname{1.4}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.vc2-rlvan.vc2.d.ci\endcsname{[$-$3.9, +1.1]}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.vc2-rlvan.vc2.d.hi\endcsname{+1.1}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.vc2-rlvan.vc2.d.lo\endcsname{$-$3.9}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.vc2-rlvan.vc2.t\endcsname{0.85}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.vc2-rlvan.vc2.t.ci\endcsname{[0.71, 1.02]}
\expandafter\def\csname N@in.mmmu.cmp.rlnotes.vc2-rlvan.vc2.t.pct\endcsname{85.1}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.f192-rlnotes.d\endcsname{$-$0.2}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.f192-rlnotes.d.abs\endcsname{0.2}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.f192-rlnotes.d.ci\endcsname{[$-$2.5, +1.9]}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.f192-rlnotes.d.hi\endcsname{+1.9}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.f192-rlnotes.d.lo\endcsname{$-$2.5}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.f192-rlnotes.match\endcsname{yes}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.f192-rlnotes.t\endcsname{0.89}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.f192-rlnotes.t.ci\endcsname{[0.77, 1.03]}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.f192-rlnotes.t.pct\endcsname{89.0}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.vc2-rlnotes.d\endcsname{$-$7.2}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.vc2-rlnotes.d.abs\endcsname{7.2}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.vc2-rlnotes.d.ci\endcsname{[$-$10.4, $-$4.2]}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.vc2-rlnotes.d.hi\endcsname{$-$4.2}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.vc2-rlnotes.d.lo\endcsname{$-$10.4}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.vc2-rlnotes.match\endcsname{no}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.vc2-rlnotes.t\endcsname{0.94}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.vc2-rlnotes.t.ci\endcsname{[0.79, 1.11]}
\expandafter\def\csname N@in.mmmu.cmp.rlvan.vc2-rlnotes.t.pct\endcsname{93.6}
\expandafter\def\csname N@in.mmmu.nnerr\endcsname{0.90}
\expandafter\def\csname N@in.mmmu.nothink.f192.acc\endcsname{88.0}
\expandafter\def\csname N@in.mmmu.nothink.f192.d\endcsname{$-$0.2}
\expandafter\def\csname N@in.mmmu.nothink.f192.d.abs\endcsname{0.2}
\expandafter\def\csname N@in.mmmu.nothink.f192.d.ci\endcsname{[$-$2.2, +1.8]}
\expandafter\def\csname N@in.mmmu.nothink.f192.d.hi\endcsname{+1.8}
\expandafter\def\csname N@in.mmmu.nothink.f192.d.lo\endcsname{$-$2.2}
\expandafter\def\csname N@in.mmmu.nothink.f192.own\endcsname{+1.2}
\expandafter\def\csname N@in.mmmu.nothink.f192.own.abs\endcsname{1.2}
\expandafter\def\csname N@in.mmmu.nothink.f192.own.ci\endcsname{[$-$0.8, +3.2]}
\expandafter\def\csname N@in.mmmu.nothink.f192.own.hi\endcsname{+3.2}
\expandafter\def\csname N@in.mmmu.nothink.f192.own.lo\endcsname{$-$0.8}
\expandafter\def\csname N@in.mmmu.nothink.f192.prompt\endcsname{22,312}
\expandafter\def\csname N@in.mmmu.nothink.f192.promptk\endcsname{22.3K}
\expandafter\def\csname N@in.mmmu.nothink.f192.t\endcsname{0.070}
\expandafter\def\csname N@in.mmmu.nothink.f192.t.ci\endcsname{[0.063, 0.077]}
\expandafter\def\csname N@in.mmmu.nothink.f192.t.pct\endcsname{7.0}
\expandafter\def\csname N@in.mmmu.nothink.f192.tok\endcsname{694}
\expandafter\def\csname N@in.mmmu.nothink.f192.vsown.t\endcsname{0.35}
\expandafter\def\csname N@in.mmmu.nothink.vc2.acc\endcsname{78.5}
\expandafter\def\csname N@in.mmmu.nothink.vc2.d\endcsname{$-$9.8}
\expandafter\def\csname N@in.mmmu.nothink.vc2.d.abs\endcsname{9.8}
\expandafter\def\csname N@in.mmmu.nothink.vc2.d.ci\endcsname{[$-$12.8, $-$6.8]}
\expandafter\def\csname N@in.mmmu.nothink.vc2.d.hi\endcsname{$-$6.8}
\expandafter\def\csname N@in.mmmu.nothink.vc2.d.lo\endcsname{$-$12.8}
\expandafter\def\csname N@in.mmmu.nothink.vc2.own\endcsname{$-$8.2}
\expandafter\def\csname N@in.mmmu.nothink.vc2.own.abs\endcsname{8.2}
\expandafter\def\csname N@in.mmmu.nothink.vc2.own.ci\endcsname{[$-$11.2, $-$5.2]}
\expandafter\def\csname N@in.mmmu.nothink.vc2.own.hi\endcsname{$-$5.2}
\expandafter\def\csname N@in.mmmu.nothink.vc2.own.lo\endcsname{$-$11.2}
\expandafter\def\csname N@in.mmmu.nothink.vc2.prompt\endcsname{22,751}
\expandafter\def\csname N@in.mmmu.nothink.vc2.promptk\endcsname{22.8K}
\expandafter\def\csname N@in.mmmu.nothink.vc2.t\endcsname{0.095}
\expandafter\def\csname N@in.mmmu.nothink.vc2.t.ci\endcsname{[0.083, 0.109]}
\expandafter\def\csname N@in.mmmu.nothink.vc2.t.pct\endcsname{9.5}
\expandafter\def\csname N@in.mmmu.nothink.vc2.tok\endcsname{944}
\expandafter\def\csname N@in.mmmu.nothink.vc2.vsown.t\endcsname{0.47}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.acc\endcsname{87.2}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.d\endcsname{$-$1.0}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.d.abs\endcsname{1.0}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.d.ci\endcsname{[$-$3.2, +1.2]}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.d.hi\endcsname{+1.2}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.d.lo\endcsname{$-$3.2}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.own\endcsname{+0.2}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.own.abs\endcsname{0.2}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.own.ci\endcsname{[$-$1.6, +2.0]}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.own.hi\endcsname{+2.0}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.own.lo\endcsname{$-$1.6}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.prompt\endcsname{22,761}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.promptk\endcsname{22.8K}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.t\endcsname{0.032}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.t.ci\endcsname{[0.026, 0.038]}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.t.pct\endcsname{3.2}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.tok\endcsname{853}
\expandafter\def\csname N@in.mmmu.rlnotes.f192.vsown.t\endcsname{0.67}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.acc\endcsname{78.4}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.d\endcsname{$-$9.9}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.d.abs\endcsname{9.9}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.d.ci\endcsname{[$-$13.4, $-$6.5]}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.d.hi\endcsname{$-$6.5}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.d.lo\endcsname{$-$13.4}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.own\endcsname{$-$8.6}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.own.abs\endcsname{8.6}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.own.ci\endcsname{[$-$12.0, $-$5.4]}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.own.hi\endcsname{$-$5.4}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.own.lo\endcsname{$-$12.0}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.prompt\endcsname{23,200}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.promptk\endcsname{23.2K}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.t\endcsname{0.038}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.t.ci\endcsname{[0.030, 0.047]}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.t.pct\endcsname{3.8}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.tok\endcsname{994}
\expandafter\def\csname N@in.mmmu.rlnotes.vc2.vsown.t\endcsname{0.80}
\expandafter\def\csname N@in.mmmu.rlvan.f192.acc\endcsname{86.8}
\expandafter\def\csname N@in.mmmu.rlvan.f192.d\endcsname{$-$1.5}
\expandafter\def\csname N@in.mmmu.rlvan.f192.d.abs\endcsname{1.5}
\expandafter\def\csname N@in.mmmu.rlvan.f192.d.ci\endcsname{[$-$3.6, +0.6]}
\expandafter\def\csname N@in.mmmu.rlvan.f192.d.hi\endcsname{+0.6}
\expandafter\def\csname N@in.mmmu.rlvan.f192.d.lo\endcsname{$-$3.6}
\expandafter\def\csname N@in.mmmu.rlvan.f192.own\endcsname{$-$1.8}
\expandafter\def\csname N@in.mmmu.rlvan.f192.own.abs\endcsname{1.8}
\expandafter\def\csname N@in.mmmu.rlvan.f192.own.ci\endcsname{[$-$4.1, +0.5]}
\expandafter\def\csname N@in.mmmu.rlvan.f192.own.hi\endcsname{+0.5}
\expandafter\def\csname N@in.mmmu.rlvan.f192.own.lo\endcsname{$-$4.1}
\expandafter\def\csname N@in.mmmu.rlvan.f192.prompt\endcsname{22,310}
\expandafter\def\csname N@in.mmmu.rlvan.f192.promptk\endcsname{22.3K}
\expandafter\def\csname N@in.mmmu.rlvan.f192.t\endcsname{0.042}
\expandafter\def\csname N@in.mmmu.rlvan.f192.t.ci\endcsname{[0.037, 0.049]}
\expandafter\def\csname N@in.mmmu.rlvan.f192.t.pct\endcsname{4.2}
\expandafter\def\csname N@in.mmmu.rlvan.f192.tok\endcsname{428}
\expandafter\def\csname N@in.mmmu.rlvan.f192.vsown.t\endcsname{0.35}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.acc\endcsname{79.8}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.d\endcsname{$-$8.5}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.d.abs\endcsname{8.5}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.d.ci\endcsname{[$-$11.9, $-$5.4]}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.d.hi\endcsname{$-$5.4}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.d.lo\endcsname{$-$11.9}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.own\endcsname{$-$8.8}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.own.abs\endcsname{8.8}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.own.ci\endcsname{[$-$12.0, $-$5.8]}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.own.hi\endcsname{$-$5.8}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.own.lo\endcsname{$-$12.0}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.prompt\endcsname{22,749}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.promptk\endcsname{22.7K}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.t\endcsname{0.044}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.t.ci\endcsname{[0.038, 0.052]}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.t.pct\endcsname{4.4}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.tok\endcsname{448}
\expandafter\def\csname N@in.mmmu.rlvan.vc2.vsown.t\endcsname{0.37}
\expandafter\def\csname N@in.rlnotes.maxloss\endcsname{1.5}
\expandafter\def\csname N@in.vh.cmp.nothink.f192-rlnotes.d\endcsname{$-$4.5}
\expandafter\def\csname N@in.vh.cmp.nothink.f192-rlnotes.d.abs\endcsname{4.5}
\expandafter\def\csname N@in.vh.cmp.nothink.f192-rlnotes.d.ci\endcsname{[$-$6.3, $-$2.7]}
\expandafter\def\csname N@in.vh.cmp.nothink.f192-rlnotes.d.hi\endcsname{$-$2.7}
\expandafter\def\csname N@in.vh.cmp.nothink.f192-rlnotes.d.lo\endcsname{$-$6.3}
\expandafter\def\csname N@in.vh.cmp.nothink.f192-rlnotes.match\endcsname{no}
\expandafter\def\csname N@in.vh.cmp.nothink.f192-rlnotes.t\endcsname{1.37}
\expandafter\def\csname N@in.vh.cmp.nothink.f192-rlnotes.t.ci\endcsname{[1.31, 1.43]}
\expandafter\def\csname N@in.vh.cmp.nothink.f192-rlnotes.t.pct\endcsname{137.3}
\expandafter\def\csname N@in.vh.cmp.nothink.vc2-rlnotes.d\endcsname{$-$6.3}
\expandafter\def\csname N@in.vh.cmp.nothink.vc2-rlnotes.d.abs\endcsname{6.3}
\expandafter\def\csname N@in.vh.cmp.nothink.vc2-rlnotes.d.ci\endcsname{[$-$8.1, $-$4.6]}
\expandafter\def\csname N@in.vh.cmp.nothink.vc2-rlnotes.d.hi\endcsname{$-$4.6}
\expandafter\def\csname N@in.vh.cmp.nothink.vc2-rlnotes.d.lo\endcsname{$-$8.1}
\expandafter\def\csname N@in.vh.cmp.nothink.vc2-rlnotes.match\endcsname{no}
\expandafter\def\csname N@in.vh.cmp.nothink.vc2-rlnotes.t\endcsname{0.98}
\expandafter\def\csname N@in.vh.cmp.nothink.vc2-rlnotes.t.ci\endcsname{[0.94, 1.02]}
\expandafter\def\csname N@in.vh.cmp.nothink.vc2-rlnotes.t.pct\endcsname{98.0}
\expandafter\def\csname N@in.vh.cmp.rlnotes.f192-rlvan.f192.d\endcsname{$-$1.4}
\expandafter\def\csname N@in.vh.cmp.rlnotes.f192-rlvan.f192.d.abs\endcsname{1.4}
\expandafter\def\csname N@in.vh.cmp.rlnotes.f192-rlvan.f192.d.ci\endcsname{[$-$3.0, +0.2]}
\expandafter\def\csname N@in.vh.cmp.rlnotes.f192-rlvan.f192.d.hi\endcsname{+0.2}
\expandafter\def\csname N@in.vh.cmp.rlnotes.f192-rlvan.f192.d.lo\endcsname{$-$3.0}
\expandafter\def\csname N@in.vh.cmp.rlnotes.f192-rlvan.f192.t\endcsname{0.81}
\expandafter\def\csname N@in.vh.cmp.rlnotes.f192-rlvan.f192.t.ci\endcsname{[0.79, 0.83]}
\expandafter\def\csname N@in.vh.cmp.rlnotes.f192-rlvan.f192.t.pct\endcsname{81.0}
\expandafter\def\csname N@in.vh.cmp.rlnotes.vc2-rlvan.vc2.d\endcsname{+0.1}
\expandafter\def\csname N@in.vh.cmp.rlnotes.vc2-rlvan.vc2.d.abs\endcsname{0.1}
\expandafter\def\csname N@in.vh.cmp.rlnotes.vc2-rlvan.vc2.d.ci\endcsname{[$-$1.6, +1.8]}
\expandafter\def\csname N@in.vh.cmp.rlnotes.vc2-rlvan.vc2.d.hi\endcsname{+1.8}
\expandafter\def\csname N@in.vh.cmp.rlnotes.vc2-rlvan.vc2.d.lo\endcsname{$-$1.6}
\expandafter\def\csname N@in.vh.cmp.rlnotes.vc2-rlvan.vc2.t\endcsname{1.07}
\expandafter\def\csname N@in.vh.cmp.rlnotes.vc2-rlvan.vc2.t.ci\endcsname{[1.03, 1.12]}
\expandafter\def\csname N@in.vh.cmp.rlnotes.vc2-rlvan.vc2.t.pct\endcsname{107.3}
\expandafter\def\csname N@in.vh.cmp.rlvan.f192-rlnotes.d\endcsname{+0.4}
\expandafter\def\csname N@in.vh.cmp.rlvan.f192-rlnotes.d.abs\endcsname{0.4}
\expandafter\def\csname N@in.vh.cmp.rlvan.f192-rlnotes.d.ci\endcsname{[$-$1.2, +2.1]}
\expandafter\def\csname N@in.vh.cmp.rlvan.f192-rlnotes.d.hi\endcsname{+2.1}
\expandafter\def\csname N@in.vh.cmp.rlvan.f192-rlnotes.d.lo\endcsname{$-$1.2}
\expandafter\def\csname N@in.vh.cmp.rlvan.f192-rlnotes.match\endcsname{yes}
\expandafter\def\csname N@in.vh.cmp.rlvan.f192-rlnotes.t\endcsname{0.99}
\expandafter\def\csname N@in.vh.cmp.rlvan.f192-rlnotes.t.ci\endcsname{[0.97, 1.02]}
\expandafter\def\csname N@in.vh.cmp.rlvan.f192-rlnotes.t.pct\endcsname{99.2}
\expandafter\def\csname N@in.vh.cmp.rlvan.vc2-rlnotes.d\endcsname{$-$1.7}
\expandafter\def\csname N@in.vh.cmp.rlvan.vc2-rlnotes.d.abs\endcsname{1.7}
\expandafter\def\csname N@in.vh.cmp.rlvan.vc2-rlnotes.d.ci\endcsname{[$-$3.5, +0.1]}
\expandafter\def\csname N@in.vh.cmp.rlvan.vc2-rlnotes.d.hi\endcsname{+0.1}
\expandafter\def\csname N@in.vh.cmp.rlvan.vc2-rlnotes.d.lo\endcsname{$-$3.5}
\expandafter\def\csname N@in.vh.cmp.rlvan.vc2-rlnotes.match\endcsname{no}
\expandafter\def\csname N@in.vh.cmp.rlvan.vc2-rlnotes.t\endcsname{0.66}
\expandafter\def\csname N@in.vh.cmp.rlvan.vc2-rlnotes.t.ci\endcsname{[0.64, 0.67]}
\expandafter\def\csname N@in.vh.cmp.rlvan.vc2-rlnotes.t.pct\endcsname{65.7}
\expandafter\def\csname N@in.vh.nnerr\endcsname{0.27}
\expandafter\def\csname N@in.vh.nothink.f192.acc\endcsname{57.9}
\expandafter\def\csname N@in.vh.nothink.f192.d\endcsname{$-$1.3}
\expandafter\def\csname N@in.vh.nothink.f192.d.abs\endcsname{1.3}
\expandafter\def\csname N@in.vh.nothink.f192.d.ci\endcsname{[$-$2.9, +0.4]}
\expandafter\def\csname N@in.vh.nothink.f192.d.hi\endcsname{+0.4}
\expandafter\def\csname N@in.vh.nothink.f192.d.lo\endcsname{$-$2.9}
\expandafter\def\csname N@in.vh.nothink.f192.own\endcsname{$-$0.7}
\expandafter\def\csname N@in.vh.nothink.f192.own.abs\endcsname{0.7}
\expandafter\def\csname N@in.vh.nothink.f192.own.ci\endcsname{[$-$2.1, +0.7]}
\expandafter\def\csname N@in.vh.nothink.f192.own.hi\endcsname{+0.7}
\expandafter\def\csname N@in.vh.nothink.f192.own.lo\endcsname{$-$2.1}
\expandafter\def\csname N@in.vh.nothink.f192.prompt\endcsname{21,271}
\expandafter\def\csname N@in.vh.nothink.f192.promptk\endcsname{21.3K}
\expandafter\def\csname N@in.vh.nothink.f192.t\endcsname{0.050}
\expandafter\def\csname N@in.vh.nothink.f192.t.ci\endcsname{[0.047, 0.053]}
\expandafter\def\csname N@in.vh.nothink.f192.t.pct\endcsname{5.0}
\expandafter\def\csname N@in.vh.nothink.f192.tok\endcsname{327}
\expandafter\def\csname N@in.vh.nothink.f192.vsown.t\endcsname{0.49}
\expandafter\def\csname N@in.vh.nothink.vc2.acc\endcsname{56.0}
\expandafter\def\csname N@in.vh.nothink.vc2.d\endcsname{$-$3.1}
\expandafter\def\csname N@in.vh.nothink.vc2.d.abs\endcsname{3.1}
\expandafter\def\csname N@in.vh.nothink.vc2.d.ci\endcsname{[$-$4.7, $-$1.5]}
\expandafter\def\csname N@in.vh.nothink.vc2.d.hi\endcsname{$-$1.5}
\expandafter\def\csname N@in.vh.nothink.vc2.d.lo\endcsname{$-$4.7}
\expandafter\def\csname N@in.vh.nothink.vc2.own\endcsname{$-$2.6}
\expandafter\def\csname N@in.vh.nothink.vc2.own.abs\endcsname{2.6}
\expandafter\def\csname N@in.vh.nothink.vc2.own.ci\endcsname{[$-$4.0, $-$1.1]}
\expandafter\def\csname N@in.vh.nothink.vc2.own.hi\endcsname{$-$1.1}
\expandafter\def\csname N@in.vh.nothink.vc2.own.lo\endcsname{$-$4.0}
\expandafter\def\csname N@in.vh.nothink.vc2.prompt\endcsname{12,281}
\expandafter\def\csname N@in.vh.nothink.vc2.promptk\endcsname{12.3K}
\expandafter\def\csname N@in.vh.nothink.vc2.t\endcsname{0.035}
\expandafter\def\csname N@in.vh.nothink.vc2.t.ci\endcsname{[0.034, 0.037]}
\expandafter\def\csname N@in.vh.nothink.vc2.t.pct\endcsname{3.5}
\expandafter\def\csname N@in.vh.nothink.vc2.tok\endcsname{349}
\expandafter\def\csname N@in.vh.nothink.vc2.vsown.t\endcsname{0.35}
\expandafter\def\csname N@in.vh.rlnotes.f192.acc\endcsname{61.3}
\expandafter\def\csname N@in.vh.rlnotes.f192.d\endcsname{+2.2}
\expandafter\def\csname N@in.vh.rlnotes.f192.d.abs\endcsname{2.2}
\expandafter\def\csname N@in.vh.rlnotes.f192.d.ci\endcsname{[+0.4, +4.0]}
\expandafter\def\csname N@in.vh.rlnotes.f192.d.hi\endcsname{+4.0}
\expandafter\def\csname N@in.vh.rlnotes.f192.d.lo\endcsname{+0.4}
\expandafter\def\csname N@in.vh.rlnotes.f192.own\endcsname{$-$1.0}
\expandafter\def\csname N@in.vh.rlnotes.f192.own.abs\endcsname{1.0}
\expandafter\def\csname N@in.vh.rlnotes.f192.own.ci\endcsname{[$-$2.2, +0.1]}
\expandafter\def\csname N@in.vh.rlnotes.f192.own.hi\endcsname{+0.1}
\expandafter\def\csname N@in.vh.rlnotes.f192.own.lo\endcsname{$-$2.2}
\expandafter\def\csname N@in.vh.rlnotes.f192.prompt\endcsname{21,720}
\expandafter\def\csname N@in.vh.rlnotes.f192.promptk\endcsname{21.7K}
\expandafter\def\csname N@in.vh.rlnotes.f192.t\endcsname{0.029}
\expandafter\def\csname N@in.vh.rlnotes.f192.t.ci\endcsname{[0.028, 0.031]}
\expandafter\def\csname N@in.vh.rlnotes.f192.t.pct\endcsname{2.9}
\expandafter\def\csname N@in.vh.rlnotes.f192.tok\endcsname{512}
\expandafter\def\csname N@in.vh.rlnotes.f192.vsown.t\endcsname{0.80}
\expandafter\def\csname N@in.vh.rlnotes.vc2.acc\endcsname{60.8}
\expandafter\def\csname N@in.vh.rlnotes.vc2.d\endcsname{+1.6}
\expandafter\def\csname N@in.vh.rlnotes.vc2.d.abs\endcsname{1.6}
\expandafter\def\csname N@in.vh.rlnotes.vc2.d.ci\endcsname{[$-$0.1, +3.4]}
\expandafter\def\csname N@in.vh.rlnotes.vc2.d.hi\endcsname{+3.4}
\expandafter\def\csname N@in.vh.rlnotes.vc2.d.lo\endcsname{$-$0.1}
\expandafter\def\csname N@in.vh.rlnotes.vc2.own\endcsname{$-$1.6}
\expandafter\def\csname N@in.vh.rlnotes.vc2.own.abs\endcsname{1.6}
\expandafter\def\csname N@in.vh.rlnotes.vc2.own.ci\endcsname{[$-$2.9, $-$0.3]}
\expandafter\def\csname N@in.vh.rlnotes.vc2.own.hi\endcsname{$-$0.3}
\expandafter\def\csname N@in.vh.rlnotes.vc2.own.lo\endcsname{$-$2.9}
\expandafter\def\csname N@in.vh.rlnotes.vc2.prompt\endcsname{12,730}
\expandafter\def\csname N@in.vh.rlnotes.vc2.promptk\endcsname{12.7K}
\expandafter\def\csname N@in.vh.rlnotes.vc2.t\endcsname{0.025}
\expandafter\def\csname N@in.vh.rlnotes.vc2.t.ci\endcsname{[0.024, 0.027]}
\expandafter\def\csname N@in.vh.rlnotes.vc2.t.pct\endcsname{2.5}
\expandafter\def\csname N@in.vh.rlnotes.vc2.tok\endcsname{511}
\expandafter\def\csname N@in.vh.rlnotes.vc2.vsown.t\endcsname{0.71}
\expandafter\def\csname N@in.vh.rlvan.f192.acc\endcsname{62.7}
\expandafter\def\csname N@in.vh.rlvan.f192.d\endcsname{+3.6}
\expandafter\def\csname N@in.vh.rlvan.f192.d.abs\endcsname{3.6}
\expandafter\def\csname N@in.vh.rlvan.f192.d.ci\endcsname{[+1.9, +5.4]}
\expandafter\def\csname N@in.vh.rlvan.f192.d.hi\endcsname{+5.4}
\expandafter\def\csname N@in.vh.rlvan.f192.d.lo\endcsname{+1.9}
\expandafter\def\csname N@in.vh.rlvan.f192.own\endcsname{+0.6}
\expandafter\def\csname N@in.vh.rlvan.f192.own.abs\endcsname{0.6}
\expandafter\def\csname N@in.vh.rlvan.f192.own.ci\endcsname{[$-$0.7, +1.9]}
\expandafter\def\csname N@in.vh.rlvan.f192.own.hi\endcsname{+1.9}
\expandafter\def\csname N@in.vh.rlvan.f192.own.lo\endcsname{$-$0.7}
\expandafter\def\csname N@in.vh.rlvan.f192.prompt\endcsname{21,269}
\expandafter\def\csname N@in.vh.rlvan.f192.promptk\endcsname{21.3K}
\expandafter\def\csname N@in.vh.rlvan.f192.t\endcsname{0.036}
\expandafter\def\csname N@in.vh.rlvan.f192.t.ci\endcsname{[0.034, 0.038]}
\expandafter\def\csname N@in.vh.rlvan.f192.t.pct\endcsname{3.6}
\expandafter\def\csname N@in.vh.rlvan.f192.tok\endcsname{236}
\expandafter\def\csname N@in.vh.rlvan.f192.vsown.t\endcsname{0.58}
\expandafter\def\csname N@in.vh.rlvan.vc2.acc\endcsname{60.6}
\expandafter\def\csname N@in.vh.rlvan.vc2.d\endcsname{+1.5}
\expandafter\def\csname N@in.vh.rlvan.vc2.d.abs\endcsname{1.5}
\expandafter\def\csname N@in.vh.rlvan.vc2.d.ci\endcsname{[$-$0.3, +3.4]}
\expandafter\def\csname N@in.vh.rlvan.vc2.d.hi\endcsname{+3.4}
\expandafter\def\csname N@in.vh.rlvan.vc2.d.lo\endcsname{$-$0.3}
\expandafter\def\csname N@in.vh.rlvan.vc2.own\endcsname{$-$1.5}
\expandafter\def\csname N@in.vh.rlvan.vc2.own.abs\endcsname{1.5}
\expandafter\def\csname N@in.vh.rlvan.vc2.own.ci\endcsname{[$-$2.8, $-$0.2]}
\expandafter\def\csname N@in.vh.rlvan.vc2.own.hi\endcsname{$-$0.2}
\expandafter\def\csname N@in.vh.rlvan.vc2.own.lo\endcsname{$-$2.8}
\expandafter\def\csname N@in.vh.rlvan.vc2.prompt\endcsname{12,279}
\expandafter\def\csname N@in.vh.rlvan.vc2.promptk\endcsname{12.3K}
\expandafter\def\csname N@in.vh.rlvan.vc2.t\endcsname{0.024}
\expandafter\def\csname N@in.vh.rlvan.vc2.t.ci\endcsname{[0.023, 0.025]}
\expandafter\def\csname N@in.vh.rlvan.vc2.t.pct\endcsname{2.4}
\expandafter\def\csname N@in.vh.rlvan.vc2.tok\endcsname{232}
\expandafter\def\csname N@in.vh.rlvan.vc2.vsown.t\endcsname{0.39}
\expandafter\def\csname N@mech.n\endcsname{199}
\expandafter\def\csname N@mech.n.c0\endcsname{0.31}
\expandafter\def\csname N@mech.n.c1024\endcsname{0.75}
\expandafter\def\csname N@mech.n.c1024.count\endcsname{113}
\expandafter\def\csname N@mech.ndep\endcsname{134}
\expandafter\def\csname N@mech.p1.gap0\endcsname{+0.3}
\expandafter\def\csname N@mech.p1.gap0.abs\endcsname{0.3}
\expandafter\def\csname N@mech.p1.gap0.ci\endcsname{[$-$0.3, +0.9]}
\expandafter\def\csname N@mech.p1.gap0.hi\endcsname{+0.9}
\expandafter\def\csname N@mech.p1.gap0.lo\endcsname{$-$0.3}
\expandafter\def\csname N@mech.p1.gap512\endcsname{$-$0.3}
\expandafter\def\csname N@mech.p1.gap512.abs\endcsname{0.3}
\expandafter\def\csname N@mech.p1.gap512.ci\endcsname{[$-$0.8, +0.2]}
\expandafter\def\csname N@mech.p1.gap512.hi\endcsname{+0.2}
\expandafter\def\csname N@mech.p1.gap512.lo\endcsname{$-$0.8}
\expandafter\def\csname N@mech.p2\endcsname{+0.5}
\expandafter\def\csname N@mech.p2.abs\endcsname{0.5}
\expandafter\def\csname N@mech.p2.ci\endcsname{[$-$0.2, +1.3]}
\expandafter\def\csname N@mech.p2.hi\endcsname{+1.3}
\expandafter\def\csname N@mech.p2.lo\endcsname{$-$0.2}
\expandafter\def\csname N@mech.p3.median\endcsname{0.29}
\expandafter\def\csname N@mech.p3.nv\endcsname{0.048}
\expandafter\def\csname N@mech.p3.orig\endcsname{0.32}
\expandafter\def\csname N@mech.p3.ratio\endcsname{0.31}
\expandafter\def\csname N@mech.p3.ratio.ci\endcsname{[0.26, 0.36]}
\expandafter\def\csname N@mech.p3.van\endcsname{0.157}
\expandafter\def\csname N@mech.p4.a\endcsname{2.14}
\expandafter\def\csname N@mech.p4.a.ci\endcsname{[1.95, 2.34]}
\expandafter\def\csname N@mech.p4.b\endcsname{$-$0.054}
\expandafter\def\csname N@mech.p4.b.ci\endcsname{[$-$0.068, $-$0.041]}
\expandafter\def\csname N@mech.p4.before\endcsname{2.28}
\expandafter\def\csname N@mech.p4.beforeother\endcsname{1.25}
\expandafter\def\csname N@mech.p4.ecited\endcsname{3.65}
\expandafter\def\csname N@mech.p4.ecited.ci\endcsname{[3.41, 3.89]}
\expandafter\def\csname N@mech.p4.eother\endcsname{1.51}
\expandafter\def\csname N@mech.p4.eother.ci\endcsname{[1.37, 1.65]}
\expandafter\def\csname N@mech.p4.kocited\endcsname{0.061}
\expandafter\def\csname N@mech.p4.korandom\endcsname{0.0004}
\expandafter\def\csname N@mech.p4.lines\endcsname{1,165}
\expandafter\def\csname N@mech.p5\endcsname{0.78}
\expandafter\def\csname N@mech.p5.ci\endcsname{[0.72, 0.83]}
\expandafter\def\csname N@mech.p5.contrib\endcsname{0.78}
\expandafter\def\csname N@mech.p5.contrib.ci\endcsname{[0.72, 0.83]}
\expandafter\def\csname N@mech.p5.did\endcsname{0.51}
\expandafter\def\csname N@mech.p5.did.ci\endcsname{[0.44, 0.58]}
\expandafter\def\csname N@mech.p5.drop\endcsname{66}
\expandafter\def\csname N@mech.p5.drop.ci\endcsname{[65, 67]}
\expandafter\def\csname N@mech.p5.fulldrop\endcsname{43}
\expandafter\def\csname N@mech.p5.fulldrop.ci\endcsname{[40, 46]}
\expandafter\def\csname N@mech.p5.mass.after\endcsname{0.11}
\expandafter\def\csname N@mech.p5.mass.notes\endcsname{0.32}
\expandafter\def\csname N@mech.p5.qratio\endcsname{1.00}
\expandafter\def\csname N@mech.p5.qratio.ci\endcsname{[0.96, 1.05]}
\expandafter\def\csname N@mech.p5.share\endcsname{100}
\expandafter\def\csname N@mech.s1.f\endcsname{0.58}
\expandafter\def\csname N@mech.s1.gs\endcsname{0.39}
\expandafter\def\csname N@mech.s1.n\endcsname{0.31}
\expandafter\def\csname N@mech.s1.qb\endcsname{0.33}
\expandafter\def\csname N@mech.s1.qbgs\endcsname{0.31}
\expandafter\def\csname N@mech.s1.qbn\endcsname{+1.5}
\expandafter\def\csname N@mech.s1.qbn.abs\endcsname{1.5}
\expandafter\def\csname N@mech.s1.qbn.ci\endcsname{[$-$2.8, +6.2]}
\expandafter\def\csname N@mech.s1.qbn.hi\endcsname{+6.2}
\expandafter\def\csname N@mech.s1.qbn.lo\endcsname{$-$2.8}
\expandafter\def\csname N@mech.tok.notes.novel\endcsname{1.06}
\expandafter\def\csname N@mech.tok.notes.repeat\endcsname{0.38}
\expandafter\def\csname N@mech.tok.van.first\endcsname{0.39}
\expandafter\def\csname N@mech.tok.van.novel\endcsname{0.34}
\expandafter\def\csname N@mech.tok.van.repeat\endcsname{0.08}
\expandafter\def\csname N@mech.tok.van.rest\endcsname{0.07}
\expandafter\def\csname N@mech.v.c0\endcsname{0.58}
\expandafter\def\csname N@mech.v.c1024\endcsname{0.77}
\expandafter\def\csname N@mech.valid.control\endcsname{0.12--0.13}
\expandafter\def\csname N@mech.valid.floor\endcsname{0.009--0.018}
\expandafter\def\csname N@mech.valid.masked\endcsname{0.010--0.014}
\expandafter\def\csname N@mech.valid.visible\endcsname{0.005}
\expandafter\def\csname N@prompt.lvb.mean\endcsname{88K}
\expandafter\def\csname N@prompt.lvb.median\endcsname{90K}
\expandafter\def\csname N@prompt.mmmu.mean\endcsname{78K}
\expandafter\def\csname N@prompt.mmmu.median\endcsname{89K}
\expandafter\def\csname N@prompt.vh.mean\endcsname{42K}
\expandafter\def\csname N@prompt.vh.median\endcsname{43K}
\expandafter\def\csname N@qual.a.hidden0\endcsname{94}
\expandafter\def\csname N@qual.a.hidden1\endcsname{240}
\expandafter\def\csname N@qual.a.mmmu.differ\endcsname{54}
\expandafter\def\csname N@qual.a.mmmu.right\endcsname{31}
\expandafter\def\csname N@qual.a.tau\endcsname{167}
\expandafter\def\csname N@qual.a.vh.differ\endcsname{256}
\expandafter\def\csname N@qual.a.vh.right\endcsname{153}
\expandafter\def\csname N@qual.b.hidden0\endcsname{69}
\expandafter\def\csname N@qual.b.hidden1\endcsname{52}
\expandafter\def\csname N@qual.b.hit.gap\endcsname{+6.4}
\expandafter\def\csname N@qual.b.hit.n\endcsname{707}
\expandafter\def\csname N@qual.b.miss.gap\endcsname{+13.0}
\expandafter\def\csname N@qual.b.miss.n\endcsname{386}
\expandafter\def\csname N@qual.b.rev\endcsname{56}
\expandafter\def\csname N@qual.b.win\endcsname{126}
\expandafter\def\csname N@qual.c.hidden0\endcsname{49}
\expandafter\def\csname N@qual.c.hidden1\endcsname{47}
\expandafter\def\csname N@qual.c.rev\endcsname{4}
\expandafter\def\csname N@qual.c.win\endcsname{21}
\expandafter\def\csname N@qvl.mmmu.blind.acc\endcsname{69.0}
\expandafter\def\csname N@qvl.mmmu.blind.d\endcsname{$-$10.3}
\expandafter\def\csname N@qvl.mmmu.blind.d.abs\endcsname{10.3}
\expandafter\def\csname N@qvl.mmmu.blind.d.ci\endcsname{[$-$15.5, $-$5.0]}
\expandafter\def\csname N@qvl.mmmu.blind.d.hi\endcsname{$-$5.0}
\expandafter\def\csname N@qvl.mmmu.blind.d.lo\endcsname{$-$15.5}
\expandafter\def\csname N@qvl.mmmu.blind.hidden\endcsname{22}
\expandafter\def\csname N@qvl.mmmu.blind.kept\endcsname{0}
\expandafter\def\csname N@qvl.mmmu.blind.t\endcsname{0.068}
\expandafter\def\csname N@qvl.mmmu.blind.tok\endcsname{1,495}
\expandafter\def\csname N@qvl.mmmu.full.acc\endcsname{79.2}
\expandafter\def\csname N@qvl.mmmu.full.tok\endcsname{1,359}
\expandafter\def\csname N@qvl.mmmu.notes.acc\endcsname{79.0}
\expandafter\def\csname N@qvl.mmmu.notes.d\endcsname{$-$0.2}
\expandafter\def\csname N@qvl.mmmu.notes.d.abs\endcsname{0.2}
\expandafter\def\csname N@qvl.mmmu.notes.d.ci\endcsname{[$-$3.2, +2.5]}
\expandafter\def\csname N@qvl.mmmu.notes.d.hi\endcsname{+2.5}
\expandafter\def\csname N@qvl.mmmu.notes.d.lo\endcsname{$-$3.2}
\expandafter\def\csname N@qvl.mmmu.notes.hidden\endcsname{238}
\expandafter\def\csname N@qvl.mmmu.notes.kept\endcsname{1}
\expandafter\def\csname N@qvl.mmmu.notes.t\endcsname{0.36}
\expandafter\def\csname N@qvl.mmmu.notes.tok\endcsname{1,776}
\expandafter\def\csname N@qvl.mmmu.posmatch.acc\endcsname{81.0}
\expandafter\def\csname N@qvl.mmmu.posmatch.d\endcsname{+1.8}
\expandafter\def\csname N@qvl.mmmu.posmatch.d.abs\endcsname{1.8}
\expandafter\def\csname N@qvl.mmmu.posmatch.d.ci\endcsname{[$-$1.5, +5.0]}
\expandafter\def\csname N@qvl.mmmu.posmatch.d.hi\endcsname{+5.0}
\expandafter\def\csname N@qvl.mmmu.posmatch.d.lo\endcsname{$-$1.5}
\expandafter\def\csname N@qvl.mmmu.posmatch.hidden\endcsname{240}
\expandafter\def\csname N@qvl.mmmu.posmatch.kept\endcsname{10}
\expandafter\def\csname N@qvl.mmmu.posmatch.t\endcsname{0.29}
\expandafter\def\csname N@qvl.mmmu.posmatch.tok\endcsname{1,458}
\expandafter\def\csname N@qvl.vh.blind.acc\endcsname{63.2}
\expandafter\def\csname N@qvl.vh.blind.d\endcsname{$-$3.9}
\expandafter\def\csname N@qvl.vh.blind.d.abs\endcsname{3.9}
\expandafter\def\csname N@qvl.vh.blind.d.ci\endcsname{[$-$6.5, $-$1.3]}
\expandafter\def\csname N@qvl.vh.blind.d.hi\endcsname{$-$1.3}
\expandafter\def\csname N@qvl.vh.blind.d.lo\endcsname{$-$6.5}
\expandafter\def\csname N@qvl.vh.blind.hidden\endcsname{22}
\expandafter\def\csname N@qvl.vh.blind.kept\endcsname{0}
\expandafter\def\csname N@qvl.vh.blind.t\endcsname{0.14}
\expandafter\def\csname N@qvl.vh.blind.tok\endcsname{1,110}
\expandafter\def\csname N@qvl.vh.full.acc\endcsname{67.0}
\expandafter\def\csname N@qvl.vh.full.tok\endcsname{709}
\expandafter\def\csname N@qvl.vh.notes.acc\endcsname{62.6}
\expandafter\def\csname N@qvl.vh.notes.d\endcsname{$-$4.4}
\expandafter\def\csname N@qvl.vh.notes.d.abs\endcsname{4.4}
\expandafter\def\csname N@qvl.vh.notes.d.ci\endcsname{[$-$7.0, $-$1.6]}
\expandafter\def\csname N@qvl.vh.notes.d.hi\endcsname{$-$1.6}
\expandafter\def\csname N@qvl.vh.notes.d.lo\endcsname{$-$7.0}
\expandafter\def\csname N@qvl.vh.notes.hidden\endcsname{342}
\expandafter\def\csname N@qvl.vh.notes.kept\endcsname{2}
\expandafter\def\csname N@qvl.vh.notes.t\endcsname{1.31}
\expandafter\def\csname N@qvl.vh.notes.tok\endcsname{1,679}
\expandafter\def\csname N@qvl.vh.posmatch.acc\endcsname{66.9}
\expandafter\def\csname N@qvl.vh.posmatch.d\endcsname{$-$0.2}
\expandafter\def\csname N@qvl.vh.posmatch.d.abs\endcsname{0.2}
\expandafter\def\csname N@qvl.vh.posmatch.d.ci\endcsname{[$-$1.6, +1.4]}
\expandafter\def\csname N@qvl.vh.posmatch.d.hi\endcsname{+1.4}
\expandafter\def\csname N@qvl.vh.posmatch.d.lo\endcsname{$-$1.6}
\expandafter\def\csname N@qvl.vh.posmatch.hidden\endcsname{306}
\expandafter\def\csname N@qvl.vh.posmatch.kept\endcsname{37}
\expandafter\def\csname N@qvl.vh.posmatch.t\endcsname{0.55}
\expandafter\def\csname N@qvl.vh.posmatch.tok\endcsname{777}
\expandafter\def\csname N@serve.bmin\endcsname{161}
\expandafter\def\csname N@serve.lvb.la0.b160\endcsname{0.17}
\expandafter\def\csname N@serve.lvb.la0.b32\endcsname{0.21}
\expandafter\def\csname N@serve.lvb.la0.b64\endcsname{0.18}
\expandafter\def\csname N@serve.lvb.la0.binf\endcsname{0.15}
\expandafter\def\csname N@serve.lvb.node\endcsname{233}
\expandafter\def\csname N@serve.mmmu.la0.b160\endcsname{0.15}
\expandafter\def\csname N@serve.mmmu.la0.b32\endcsname{0.22}
\expandafter\def\csname N@serve.mmmu.la0.b64\endcsname{0.18}
\expandafter\def\csname N@serve.mmmu.la0.binf\endcsname{0.13}
\expandafter\def\csname N@serve.mmmu.node\endcsname{261}
\expandafter\def\csname N@serve.open.la0.max\endcsname{0.9}
\expandafter\def\csname N@serve.open.larl.max\endcsname{0.0}
\expandafter\def\csname N@serve.vh.la0.b160\endcsname{0.14}
\expandafter\def\csname N@serve.vh.la0.b32\endcsname{0.21}
\expandafter\def\csname N@serve.vh.la0.b64\endcsname{0.17}
\expandafter\def\csname N@serve.vh.la0.binf\endcsname{0.12}
\expandafter\def\csname N@serve.vh.node\endcsname{465}
\expandafter\def\csname N@serve.wstep.ms\endcsname{9.6}
\expandafter\def\csname N@tab1.mmmu.underline\endcsname{fixed-512}
\expandafter\def\csname N@tab1.vh.underline\endcsname{notes}
\expandafter\def\csname N@test.lvb.H1.d\endcsname{$-$2.8}
\expandafter\def\csname N@test.lvb.H1.d.abs\endcsname{2.8}
\expandafter\def\csname N@test.lvb.H1.d.ci\endcsname{[$-$4.9, $-$0.7]}
\expandafter\def\csname N@test.lvb.H1.d.hi\endcsname{$-$0.7}
\expandafter\def\csname N@test.lvb.H1.d.lo\endcsname{$-$4.9}
\expandafter\def\csname N@test.lvb.H1.pass\endcsname{fail}
\expandafter\def\csname N@test.lvb.H1.t\endcsname{0.023}
\expandafter\def\csname N@test.lvb.H1.t.ci\endcsname{[0.020, 0.026]}
\expandafter\def\csname N@test.lvb.H1.t.pct\endcsname{2.3}
\expandafter\def\csname N@test.lvb.H3.d\endcsname{+0.1}
\expandafter\def\csname N@test.lvb.H3.d.abs\endcsname{0.1}
\expandafter\def\csname N@test.lvb.H3.d.ci\endcsname{[$-$1.9, +2.1]}
\expandafter\def\csname N@test.lvb.H3.d.hi\endcsname{+2.1}
\expandafter\def\csname N@test.lvb.H3.d.lo\endcsname{$-$1.9}
\expandafter\def\csname N@test.lvb.H3.pass\endcsname{pass}
\expandafter\def\csname N@test.lvb.H3.t\endcsname{0.43}
\expandafter\def\csname N@test.lvb.H3.t.ci\endcsname{[0.42, 0.44]}
\expandafter\def\csname N@test.lvb.H3.t.pct\endcsname{43.3}
\expandafter\def\csname N@test.lvb.basenotes.acc\endcsname{65.5}
\expandafter\def\csname N@test.lvb.basenotes.d\endcsname{$-$1.0}
\expandafter\def\csname N@test.lvb.basenotes.d.abs\endcsname{1.0}
\expandafter\def\csname N@test.lvb.basenotes.d.ci\endcsname{[$-$3.0, +1.0]}
\expandafter\def\csname N@test.lvb.basenotes.d.hi\endcsname{+1.0}
\expandafter\def\csname N@test.lvb.basenotes.d.lo\endcsname{$-$3.0}
\expandafter\def\csname N@test.lvb.basenotes.t\endcsname{0.16}
\expandafter\def\csname N@test.lvb.basenotes.t.ci\endcsname{[0.12, 0.20]}
\expandafter\def\csname N@test.lvb.basenotes.t.pct\endcsname{15.5}
\expandafter\def\csname N@test.lvb.basenotes.tok\endcsname{1,160}
\expandafter\def\csname N@test.lvb.basevan.acc\endcsname{66.5}
\expandafter\def\csname N@test.lvb.basevan.tok\endcsname{2,880}
\expandafter\def\csname N@test.lvb.nothink.acc\endcsname{66.3}
\expandafter\def\csname N@test.lvb.nothink.d\endcsname{$-$0.3}
\expandafter\def\csname N@test.lvb.nothink.d.abs\endcsname{0.3}
\expandafter\def\csname N@test.lvb.nothink.d.ci\endcsname{[$-$2.3, +1.7]}
\expandafter\def\csname N@test.lvb.nothink.d.hi\endcsname{+1.7}
\expandafter\def\csname N@test.lvb.nothink.d.lo\endcsname{$-$2.3}
\expandafter\def\csname N@test.lvb.nothink.t\endcsname{0.060}
\expandafter\def\csname N@test.lvb.nothink.t.ci\endcsname{[0.053, 0.068]}
\expandafter\def\csname N@test.lvb.nothink.t.pct\endcsname{6.0}
\expandafter\def\csname N@test.lvb.nothink.tok\endcsname{182}
\expandafter\def\csname N@test.lvb.q\endcsname{1,095}
\expandafter\def\csname N@test.lvb.reads.rlnotes.rlvan.pct\endcsname{34}
\expandafter\def\csname N@test.lvb.rlnotes.acc\endcsname{63.7}
\expandafter\def\csname N@test.lvb.rlnotes.d\endcsname{$-$2.8}
\expandafter\def\csname N@test.lvb.rlnotes.d.abs\endcsname{2.8}
\expandafter\def\csname N@test.lvb.rlnotes.d.ci\endcsname{[$-$4.9, $-$0.7]}
\expandafter\def\csname N@test.lvb.rlnotes.d.hi\endcsname{$-$0.7}
\expandafter\def\csname N@test.lvb.rlnotes.d.lo\endcsname{$-$4.9}
\expandafter\def\csname N@test.lvb.rlnotes.t\endcsname{0.023}
\expandafter\def\csname N@test.lvb.rlnotes.t.ci\endcsname{[0.020, 0.026]}
\expandafter\def\csname N@test.lvb.rlnotes.t.pct\endcsname{2.3}
\expandafter\def\csname N@test.lvb.rlnotes.tok\endcsname{275}
\expandafter\def\csname N@test.lvb.rlvan.acc\endcsname{63.6}
\expandafter\def\csname N@test.lvb.rlvan.d\endcsname{$-$2.9}
\expandafter\def\csname N@test.lvb.rlvan.d.abs\endcsname{2.9}
\expandafter\def\csname N@test.lvb.rlvan.d.ci\endcsname{[$-$5.2, $-$0.8]}
\expandafter\def\csname N@test.lvb.rlvan.d.hi\endcsname{$-$0.8}
\expandafter\def\csname N@test.lvb.rlvan.d.lo\endcsname{$-$5.2}
\expandafter\def\csname N@test.lvb.rlvan.t\endcsname{0.052}
\expandafter\def\csname N@test.lvb.rlvan.t.ci\endcsname{[0.047, 0.059]}
\expandafter\def\csname N@test.lvb.rlvan.t.pct\endcsname{5.2}
\expandafter\def\csname N@test.lvb.rlvan.tok\endcsname{159}
\expandafter\def\csname N@test.lvb.sftnotes.acc\endcsname{64.4}
\expandafter\def\csname N@test.lvb.sftnotes.d\endcsname{$-$2.1}
\expandafter\def\csname N@test.lvb.sftnotes.d.abs\endcsname{2.1}
\expandafter\def\csname N@test.lvb.sftnotes.d.ci\endcsname{[$-$4.2, $-$0.1]}
\expandafter\def\csname N@test.lvb.sftnotes.d.hi\endcsname{$-$0.1}
\expandafter\def\csname N@test.lvb.sftnotes.d.lo\endcsname{$-$4.2}
\expandafter\def\csname N@test.lvb.sftnotes.t\endcsname{0.16}
\expandafter\def\csname N@test.lvb.sftnotes.t.ci\endcsname{[0.12, 0.20]}
\expandafter\def\csname N@test.lvb.sftnotes.t.pct\endcsname{15.6}
\expandafter\def\csname N@test.lvb.sftnotes.tok\endcsname{1,196}
\expandafter\def\csname N@test.lvb.sftvan.acc\endcsname{65.4}
\expandafter\def\csname N@test.lvb.sftvan.d\endcsname{$-$1.1}
\expandafter\def\csname N@test.lvb.sftvan.d.abs\endcsname{1.1}
\expandafter\def\csname N@test.lvb.sftvan.d.ci\endcsname{[$-$2.8, +0.5]}
\expandafter\def\csname N@test.lvb.sftvan.d.hi\endcsname{+0.5}
\expandafter\def\csname N@test.lvb.sftvan.d.lo\endcsname{$-$2.8}
\expandafter\def\csname N@test.lvb.sftvan.t\endcsname{0.95}
\expandafter\def\csname N@test.lvb.sftvan.t.ci\endcsname{[0.89, 1.02]}
\expandafter\def\csname N@test.lvb.sftvan.t.pct\endcsname{95.2}
\expandafter\def\csname N@test.lvb.sftvan.tok\endcsname{2,750}
\expandafter\def\csname N@test.lvb.stepreads.rlnotes.rlvan.x\endcsname{5.1}
\expandafter\def\csname N@test.lvb.sub.basenotes\endcsname{33.3}
\expandafter\def\csname N@test.lvb.sub.basevan\endcsname{58.1}
\expandafter\def\csname N@test.lvb.sub.gain\endcsname{28.0}
\expandafter\def\csname N@test.lvb.sub.nothink\endcsname{30.1}
\expandafter\def\csname N@test.lvb.sub.q\endcsname{93}
\expandafter\def\csname N@test.lvb.sub.retain.rlnotes\endcsname{31}
\expandafter\def\csname N@test.lvb.sub.retain.rlvan\endcsname{23}
\expandafter\def\csname N@test.lvb.sub.rlnotes\endcsname{38.7}
\expandafter\def\csname N@test.lvb.sub.rlvan\endcsname{36.6}
\expandafter\def\csname N@test.lvb.sub.sftnotes\endcsname{43.0}
\expandafter\def\csname N@test.lvb.sub.sftvan\endcsname{53.8}
\expandafter\def\csname N@test.lvb.tokratio.basevan.rlnotes\endcsname{10.5}
\expandafter\def\csname N@test.lvb.tokratio.rlnotes.rlvan\endcsname{1.7}
\expandafter\def\csname N@test.lvb.videos\endcsname{73}
\expandafter\def\csname N@test.lvb.vsnothink.d\endcsname{$-$2.6}
\expandafter\def\csname N@test.lvb.vsnothink.d.abs\endcsname{2.6}
\expandafter\def\csname N@test.lvb.vsnothink.d.ci\endcsname{[$-$4.7, $-$0.5]}
\expandafter\def\csname N@test.lvb.vsnothink.d.hi\endcsname{$-$0.5}
\expandafter\def\csname N@test.lvb.vsnothink.d.lo\endcsname{$-$4.7}
\expandafter\def\csname N@test.lvb.vsnothink.t\endcsname{0.38}
\expandafter\def\csname N@test.lvb.vsnothink.t.ci\endcsname{[0.34, 0.43]}
\expandafter\def\csname N@test.lvb.vsnothink.t.pct\endcsname{38.0}
\expandafter\def\csname N@test.mmmu.H1.d\endcsname{$-$1.2}
\expandafter\def\csname N@test.mmmu.H1.d.abs\endcsname{1.2}
\expandafter\def\csname N@test.mmmu.H1.d.ci\endcsname{[$-$3.5, +1.1]}
\expandafter\def\csname N@test.mmmu.H1.d.hi\endcsname{+1.1}
\expandafter\def\csname N@test.mmmu.H1.d.lo\endcsname{$-$3.5}
\expandafter\def\csname N@test.mmmu.H1.pass\endcsname{fail}
\expandafter\def\csname N@test.mmmu.H1.t\endcsname{0.047}
\expandafter\def\csname N@test.mmmu.H1.t.ci\endcsname{[0.039, 0.058]}
\expandafter\def\csname N@test.mmmu.H1.t.pct\endcsname{4.7}
\expandafter\def\csname N@test.mmmu.H3.d\endcsname{$-$1.5}
\expandafter\def\csname N@test.mmmu.H3.d.abs\endcsname{1.5}
\expandafter\def\csname N@test.mmmu.H3.d.ci\endcsname{[$-$3.6, +0.5]}
\expandafter\def\csname N@test.mmmu.H3.d.hi\endcsname{+0.5}
\expandafter\def\csname N@test.mmmu.H3.d.lo\endcsname{$-$3.6}
\expandafter\def\csname N@test.mmmu.H3.pass\endcsname{fail}
\expandafter\def\csname N@test.mmmu.H3.t\endcsname{0.40}
\expandafter\def\csname N@test.mmmu.H3.t.ci\endcsname{[0.34, 0.46]}
\expandafter\def\csname N@test.mmmu.H3.t.pct\endcsname{39.7}
\expandafter\def\csname N@test.mmmu.basenotes.acc\endcsname{86.8}
\expandafter\def\csname N@test.mmmu.basenotes.d\endcsname{$-$1.5}
\expandafter\def\csname N@test.mmmu.basenotes.d.abs\endcsname{1.5}
\expandafter\def\csname N@test.mmmu.basenotes.d.ci\endcsname{[$-$3.5, +0.5]}
\expandafter\def\csname N@test.mmmu.basenotes.d.hi\endcsname{+0.5}
\expandafter\def\csname N@test.mmmu.basenotes.d.lo\endcsname{$-$3.5}
\expandafter\def\csname N@test.mmmu.basenotes.t\endcsname{0.13}
\expandafter\def\csname N@test.mmmu.basenotes.t.ci\endcsname{[0.11, 0.14]}
\expandafter\def\csname N@test.mmmu.basenotes.t.pct\endcsname{12.7}
\expandafter\def\csname N@test.mmmu.basenotes.tok\endcsname{1,729}
\expandafter\def\csname N@test.mmmu.basevan.acc\endcsname{88.2}
\expandafter\def\csname N@test.mmmu.basevan.tok\endcsname{3,245}
\expandafter\def\csname N@test.mmmu.nothink.acc\endcsname{86.8}
\expandafter\def\csname N@test.mmmu.nothink.d\endcsname{$-$1.5}
\expandafter\def\csname N@test.mmmu.nothink.d.abs\endcsname{1.5}
\expandafter\def\csname N@test.mmmu.nothink.d.ci\endcsname{[$-$3.5, +0.5]}
\expandafter\def\csname N@test.mmmu.nothink.d.hi\endcsname{+0.5}
\expandafter\def\csname N@test.mmmu.nothink.d.lo\endcsname{$-$3.5}
\expandafter\def\csname N@test.mmmu.nothink.t\endcsname{0.20}
\expandafter\def\csname N@test.mmmu.nothink.t.ci\endcsname{[0.18, 0.22]}
\expandafter\def\csname N@test.mmmu.nothink.t.pct\endcsname{20.0}
\expandafter\def\csname N@test.mmmu.nothink.tok\endcsname{685}
\expandafter\def\csname N@test.mmmu.q\endcsname{400}
\expandafter\def\csname N@test.mmmu.reads.rlnotes.rlvan.pct\endcsname{27}
\expandafter\def\csname N@test.mmmu.rlnotes.acc\endcsname{87.0}
\expandafter\def\csname N@test.mmmu.rlnotes.d\endcsname{$-$1.2}
\expandafter\def\csname N@test.mmmu.rlnotes.d.abs\endcsname{1.2}
\expandafter\def\csname N@test.mmmu.rlnotes.d.ci\endcsname{[$-$3.5, +1.1]}
\expandafter\def\csname N@test.mmmu.rlnotes.d.hi\endcsname{+1.1}
\expandafter\def\csname N@test.mmmu.rlnotes.d.lo\endcsname{$-$3.5}
\expandafter\def\csname N@test.mmmu.rlnotes.t\endcsname{0.047}
\expandafter\def\csname N@test.mmmu.rlnotes.t.ci\endcsname{[0.039, 0.058]}
\expandafter\def\csname N@test.mmmu.rlnotes.t.pct\endcsname{4.7}
\expandafter\def\csname N@test.mmmu.rlnotes.tok\endcsname{836}
\expandafter\def\csname N@test.mmmu.rlvan.acc\endcsname{88.5}
\expandafter\def\csname N@test.mmmu.rlvan.d\endcsname{+0.2}
\expandafter\def\csname N@test.mmmu.rlvan.d.abs\endcsname{0.2}
\expandafter\def\csname N@test.mmmu.rlvan.d.ci\endcsname{[$-$1.8, +2.2]}
\expandafter\def\csname N@test.mmmu.rlvan.d.hi\endcsname{+2.2}
\expandafter\def\csname N@test.mmmu.rlvan.d.lo\endcsname{$-$1.8}
\expandafter\def\csname N@test.mmmu.rlvan.t\endcsname{0.12}
\expandafter\def\csname N@test.mmmu.rlvan.t.ci\endcsname{[0.10, 0.14]}
\expandafter\def\csname N@test.mmmu.rlvan.t.pct\endcsname{11.9}
\expandafter\def\csname N@test.mmmu.rlvan.tok\endcsname{424}
\expandafter\def\csname N@test.mmmu.sftnotes.acc\endcsname{87.4}
\expandafter\def\csname N@test.mmmu.sftnotes.d\endcsname{$-$0.9}
\expandafter\def\csname N@test.mmmu.sftnotes.d.abs\endcsname{0.9}
\expandafter\def\csname N@test.mmmu.sftnotes.d.ci\endcsname{[$-$2.8, +1.0]}
\expandafter\def\csname N@test.mmmu.sftnotes.d.hi\endcsname{+1.0}
\expandafter\def\csname N@test.mmmu.sftnotes.d.lo\endcsname{$-$2.8}
\expandafter\def\csname N@test.mmmu.sftnotes.t\endcsname{0.13}
\expandafter\def\csname N@test.mmmu.sftnotes.t.ci\endcsname{[0.12, 0.14]}
\expandafter\def\csname N@test.mmmu.sftnotes.t.pct\endcsname{12.8}
\expandafter\def\csname N@test.mmmu.sftnotes.tok\endcsname{1,752}
\expandafter\def\csname N@test.mmmu.sftvan.acc\endcsname{87.2}
\expandafter\def\csname N@test.mmmu.sftvan.d\endcsname{$-$1.0}
\expandafter\def\csname N@test.mmmu.sftvan.d.abs\endcsname{1.0}
\expandafter\def\csname N@test.mmmu.sftvan.d.ci\endcsname{[$-$2.6, +0.5]}
\expandafter\def\csname N@test.mmmu.sftvan.d.hi\endcsname{+0.5}
\expandafter\def\csname N@test.mmmu.sftvan.d.lo\endcsname{$-$2.6}
\expandafter\def\csname N@test.mmmu.sftvan.t\endcsname{0.95}
\expandafter\def\csname N@test.mmmu.sftvan.t.ci\endcsname{[0.90, 1.02]}
\expandafter\def\csname N@test.mmmu.sftvan.t.pct\endcsname{95.2}
\expandafter\def\csname N@test.mmmu.sftvan.tok\endcsname{3,130}
\expandafter\def\csname N@test.mmmu.stepreads.rlnotes.rlvan.x\endcsname{7.4}
\expandafter\def\csname N@test.mmmu.sub.basenotes\endcsname{62.5}
\expandafter\def\csname N@test.mmmu.sub.basevan\endcsname{62.5}
\expandafter\def\csname N@test.mmmu.sub.gain\endcsname{20.8}
\expandafter\def\csname N@test.mmmu.sub.nothink\endcsname{41.7}
\expandafter\def\csname N@test.mmmu.sub.q\endcsname{24}
\expandafter\def\csname N@test.mmmu.sub.retain.rlnotes\endcsname{120}
\expandafter\def\csname N@test.mmmu.sub.retain.rlvan\endcsname{20}
\expandafter\def\csname N@test.mmmu.sub.rlnotes\endcsname{66.7}
\expandafter\def\csname N@test.mmmu.sub.rlvan\endcsname{45.8}
\expandafter\def\csname N@test.mmmu.sub.sftnotes\endcsname{45.8}
\expandafter\def\csname N@test.mmmu.sub.sftvan\endcsname{62.5}
\expandafter\def\csname N@test.mmmu.tokratio.basevan.rlnotes\endcsname{3.9}
\expandafter\def\csname N@test.mmmu.tokratio.rlnotes.rlvan\endcsname{2.0}
\expandafter\def\csname N@test.mmmu.videos\endcsname{200}
\expandafter\def\csname N@test.mmmu.vsnothink.d\endcsname{+0.2}
\expandafter\def\csname N@test.mmmu.vsnothink.d.abs\endcsname{0.2}
\expandafter\def\csname N@test.mmmu.vsnothink.d.ci\endcsname{[$-$2.2, +2.8]}
\expandafter\def\csname N@test.mmmu.vsnothink.d.hi\endcsname{+2.8}
\expandafter\def\csname N@test.mmmu.vsnothink.d.lo\endcsname{$-$2.2}
\expandafter\def\csname N@test.mmmu.vsnothink.t\endcsname{0.24}
\expandafter\def\csname N@test.mmmu.vsnothink.t.ci\endcsname{[0.20, 0.28]}
\expandafter\def\csname N@test.mmmu.vsnothink.t.pct\endcsname{23.7}
\expandafter\def\csname N@test.pooled.H1.d\endcsname{+0.7}
\expandafter\def\csname N@test.pooled.H1.d.abs\endcsname{0.7}
\expandafter\def\csname N@test.pooled.H1.d.ci\endcsname{[$-$0.5, +1.9]}
\expandafter\def\csname N@test.pooled.H1.d.hi\endcsname{+1.9}
\expandafter\def\csname N@test.pooled.H1.d.lo\endcsname{$-$0.5}
\expandafter\def\csname N@test.pooled.H1.t\endcsname{0.032}
\expandafter\def\csname N@test.pooled.H1.t.ci\endcsname{[0.030, 0.035]}
\expandafter\def\csname N@test.pooled.H1.t.pct\endcsname{3.2}
\expandafter\def\csname N@test.pooled.H3.d\endcsname{0.0}
\expandafter\def\csname N@test.pooled.H3.d.abs\endcsname{0.0}
\expandafter\def\csname N@test.pooled.H3.d.ci\endcsname{[$-$1.1, +1.0]}
\expandafter\def\csname N@test.pooled.H3.d.hi\endcsname{+1.0}
\expandafter\def\csname N@test.pooled.H3.d.lo\endcsname{$-$1.1}
\expandafter\def\csname N@test.pooled.H3.t\endcsname{0.49}
\expandafter\def\csname N@test.pooled.H3.t.ci\endcsname{[0.47, 0.51]}
\expandafter\def\csname N@test.pooled.H3.t.pct\endcsname{48.5}
\expandafter\def\csname N@test.vh.H1.d\endcsname{+3.2}
\expandafter\def\csname N@test.vh.H1.d.abs\endcsname{3.2}
\expandafter\def\csname N@test.vh.H1.d.ci\endcsname{[+1.5, +4.9]}
\expandafter\def\csname N@test.vh.H1.d.hi\endcsname{+4.9}
\expandafter\def\csname N@test.vh.H1.d.lo\endcsname{+1.5}
\expandafter\def\csname N@test.vh.H1.pass\endcsname{pass}
\expandafter\def\csname N@test.vh.H1.t\endcsname{0.036}
\expandafter\def\csname N@test.vh.H1.t.ci\endcsname{[0.035, 0.038]}
\expandafter\def\csname N@test.vh.H1.t.pct\endcsname{3.6}
\expandafter\def\csname N@test.vh.H3.d\endcsname{+0.2}
\expandafter\def\csname N@test.vh.H3.d.abs\endcsname{0.2}
\expandafter\def\csname N@test.vh.H3.d.ci\endcsname{[$-$1.3, +1.7]}
\expandafter\def\csname N@test.vh.H3.d.hi\endcsname{+1.7}
\expandafter\def\csname N@test.vh.H3.d.lo\endcsname{$-$1.3}
\expandafter\def\csname N@test.vh.H3.pass\endcsname{pass}
\expandafter\def\csname N@test.vh.H3.t\endcsname{0.59}
\expandafter\def\csname N@test.vh.H3.t.ci\endcsname{[0.57, 0.60]}
\expandafter\def\csname N@test.vh.H3.t.pct\endcsname{58.7}
\expandafter\def\csname N@test.vh.basenotes.acc\endcsname{57.5}
\expandafter\def\csname N@test.vh.basenotes.d\endcsname{$-$1.6}
\expandafter\def\csname N@test.vh.basenotes.d.abs\endcsname{1.6}
\expandafter\def\csname N@test.vh.basenotes.d.ci\endcsname{[$-$3.0, $-$0.2]}
\expandafter\def\csname N@test.vh.basenotes.d.hi\endcsname{$-$0.2}
\expandafter\def\csname N@test.vh.basenotes.d.lo\endcsname{$-$3.0}
\expandafter\def\csname N@test.vh.basenotes.t\endcsname{0.12}
\expandafter\def\csname N@test.vh.basenotes.t.ci\endcsname{[0.11, 0.13]}
\expandafter\def\csname N@test.vh.basenotes.t.pct\endcsname{11.9}
\expandafter\def\csname N@test.vh.basenotes.tok\endcsname{1,357}
\expandafter\def\csname N@test.vh.basevan.acc\endcsname{59.1}
\expandafter\def\csname N@test.vh.basevan.tok\endcsname{3,564}
\expandafter\def\csname N@test.vh.nothink.acc\endcsname{58.6}
\expandafter\def\csname N@test.vh.nothink.d\endcsname{$-$0.5}
\expandafter\def\csname N@test.vh.nothink.d.abs\endcsname{0.5}
\expandafter\def\csname N@test.vh.nothink.d.ci\endcsname{[$-$2.1, +1.1]}
\expandafter\def\csname N@test.vh.nothink.d.hi\endcsname{+1.1}
\expandafter\def\csname N@test.vh.nothink.d.lo\endcsname{$-$2.1}
\expandafter\def\csname N@test.vh.nothink.t\endcsname{0.10}
\expandafter\def\csname N@test.vh.nothink.t.ci\endcsname{[0.10, 0.11]}
\expandafter\def\csname N@test.vh.nothink.t.pct\endcsname{10.2}
\expandafter\def\csname N@test.vh.nothink.tok\endcsname{390}
\expandafter\def\csname N@test.vh.q\endcsname{1,837}
\expandafter\def\csname N@test.vh.reads.rlnotes.rlvan.pct\endcsname{35}
\expandafter\def\csname N@test.vh.rlnotes.acc\endcsname{62.3}
\expandafter\def\csname N@test.vh.rlnotes.d\endcsname{+3.2}
\expandafter\def\csname N@test.vh.rlnotes.d.abs\endcsname{3.2}
\expandafter\def\csname N@test.vh.rlnotes.d.ci\endcsname{[+1.5, +4.9]}
\expandafter\def\csname N@test.vh.rlnotes.d.hi\endcsname{+4.9}
\expandafter\def\csname N@test.vh.rlnotes.d.lo\endcsname{+1.5}
\expandafter\def\csname N@test.vh.rlnotes.t\endcsname{0.036}
\expandafter\def\csname N@test.vh.rlnotes.t.ci\endcsname{[0.035, 0.038]}
\expandafter\def\csname N@test.vh.rlnotes.t.pct\endcsname{3.6}
\expandafter\def\csname N@test.vh.rlnotes.tok\endcsname{499}
\expandafter\def\csname N@test.vh.rlvan.acc\endcsname{62.1}
\expandafter\def\csname N@test.vh.rlvan.d\endcsname{+3.0}
\expandafter\def\csname N@test.vh.rlvan.d.abs\endcsname{3.0}
\expandafter\def\csname N@test.vh.rlvan.d.ci\endcsname{[+1.3, +4.7]}
\expandafter\def\csname N@test.vh.rlvan.d.hi\endcsname{+4.7}
\expandafter\def\csname N@test.vh.rlvan.d.lo\endcsname{+1.3}
\expandafter\def\csname N@test.vh.rlvan.t\endcsname{0.062}
\expandafter\def\csname N@test.vh.rlvan.t.ci\endcsname{[0.059, 0.064]}
\expandafter\def\csname N@test.vh.rlvan.t.pct\endcsname{6.2}
\expandafter\def\csname N@test.vh.rlvan.tok\endcsname{232}
\expandafter\def\csname N@test.vh.sftnotes.acc\endcsname{57.7}
\expandafter\def\csname N@test.vh.sftnotes.d\endcsname{$-$1.4}
\expandafter\def\csname N@test.vh.sftnotes.d.abs\endcsname{1.4}
\expandafter\def\csname N@test.vh.sftnotes.d.ci\endcsname{[$-$2.8, 0.0]}
\expandafter\def\csname N@test.vh.sftnotes.d.hi\endcsname{0.0}
\expandafter\def\csname N@test.vh.sftnotes.d.lo\endcsname{$-$2.8}
\expandafter\def\csname N@test.vh.sftnotes.t\endcsname{0.13}
\expandafter\def\csname N@test.vh.sftnotes.t.ci\endcsname{[0.13, 0.14]}
\expandafter\def\csname N@test.vh.sftnotes.t.pct\endcsname{13.2}
\expandafter\def\csname N@test.vh.sftnotes.tok\endcsname{1,552}
\expandafter\def\csname N@test.vh.sftvan.acc\endcsname{58.9}
\expandafter\def\csname N@test.vh.sftvan.d\endcsname{$-$0.2}
\expandafter\def\csname N@test.vh.sftvan.d.abs\endcsname{0.2}
\expandafter\def\csname N@test.vh.sftvan.d.ci\endcsname{[$-$1.6, +1.2]}
\expandafter\def\csname N@test.vh.sftvan.d.hi\endcsname{+1.2}
\expandafter\def\csname N@test.vh.sftvan.d.lo\endcsname{$-$1.6}
\expandafter\def\csname N@test.vh.sftvan.t\endcsname{0.93}
\expandafter\def\csname N@test.vh.sftvan.t.ci\endcsname{[0.90, 0.96]}
\expandafter\def\csname N@test.vh.sftvan.t.pct\endcsname{92.8}
\expandafter\def\csname N@test.vh.sftvan.tok\endcsname{3,306}
\expandafter\def\csname N@test.vh.stepreads.rlnotes.rlvan.x\endcsname{6.1}
\expandafter\def\csname N@test.vh.sub.basenotes\endcsname{50.8}
\expandafter\def\csname N@test.vh.sub.basevan\endcsname{59.3}
\expandafter\def\csname N@test.vh.sub.gain\endcsname{20.6}
\expandafter\def\csname N@test.vh.sub.nothink\endcsname{38.7}
\expandafter\def\csname N@test.vh.sub.q\endcsname{199}
\expandafter\def\csname N@test.vh.sub.retain.rlnotes\endcsname{73}
\expandafter\def\csname N@test.vh.sub.retain.rlvan\endcsname{83}
\expandafter\def\csname N@test.vh.sub.rlnotes\endcsname{53.8}
\expandafter\def\csname N@test.vh.sub.rlvan\endcsname{55.8}
\expandafter\def\csname N@test.vh.sub.sftnotes\endcsname{53.3}
\expandafter\def\csname N@test.vh.sub.sftvan\endcsname{59.3}
\expandafter\def\csname N@test.vh.tokratio.basevan.rlnotes\endcsname{7.1}
\expandafter\def\csname N@test.vh.tokratio.rlnotes.rlvan\endcsname{2.1}
\expandafter\def\csname N@test.vh.videos\endcsname{270}
\expandafter\def\csname N@test.vh.vsnothink.d\endcsname{+3.8}
\expandafter\def\csname N@test.vh.vsnothink.d.abs\endcsname{3.8}
\expandafter\def\csname N@test.vh.vsnothink.d.ci\endcsname{[+2.1, +5.4]}
\expandafter\def\csname N@test.vh.vsnothink.d.hi\endcsname{+5.4}
\expandafter\def\csname N@test.vh.vsnothink.d.lo\endcsname{+2.1}
\expandafter\def\csname N@test.vh.vsnothink.t\endcsname{0.35}
\expandafter\def\csname N@test.vh.vsnothink.t.ci\endcsname{[0.34, 0.37]}
\expandafter\def\csname N@test.vh.vsnothink.t.pct\endcsname{35.4}
\expandafter\def\csname N@train.decodereads.ratio.last\endcsname{0.39}
\expandafter\def\csname N@train.notes.correct.first\endcsname{0.368}
\expandafter\def\csname N@train.notes.correct.last\endcsname{0.716}
\expandafter\def\csname N@train.notes.over.first\endcsname{32}
\expandafter\def\csname N@train.notes.over.last\endcsname{18}
\expandafter\def\csname N@train.notes.resp.first\endcsname{941}
\expandafter\def\csname N@train.notes.resp.last\endcsname{299}
\expandafter\def\csname N@train.notes.visible.last\endcsname{52}
\expandafter\def\csname N@train.vanilla.correct.first\endcsname{0.346}
\expandafter\def\csname N@train.vanilla.correct.last\endcsname{0.741}
\expandafter\def\csname N@train.vanilla.over.first\endcsname{86}
\expandafter\def\csname N@train.vanilla.over.last\endcsname{16}
\expandafter\def\csname N@train.vanilla.resp.first\endcsname{2,197}
\expandafter\def\csname N@train.vanilla.resp.last\endcsname{152}
\expandafter\def\csname N@train.vanilla.visible.last\endcsname{152}
\expandafter\def\csname N@x.mmmu.blind-vanilla\endcsname{$-$16.8}
\expandafter\def\csname N@x.mmmu.blind-vanilla.abs\endcsname{16.8}
\expandafter\def\csname N@x.mmmu.blind-vanilla.ci\endcsname{[$-$22.5, $-$11.0]}
\expandafter\def\csname N@x.mmmu.blind-vanilla.hi\endcsname{$-$11.0}
\expandafter\def\csname N@x.mmmu.blind-vanilla.lo\endcsname{$-$22.5}
\expandafter\def\csname N@x.mmmu.fixed-512-vanilla\endcsname{0.0}
\expandafter\def\csname N@x.mmmu.fixed-512-vanilla.abs\endcsname{0.0}
\expandafter\def\csname N@x.mmmu.fixed-512-vanilla.ci\endcsname{[$-$2.0, +2.0]}
\expandafter\def\csname N@x.mmmu.fixed-512-vanilla.hi\endcsname{+2.0}
\expandafter\def\csname N@x.mmmu.fixed-512-vanilla.lo\endcsname{$-$2.0}
\expandafter\def\csname N@x.mmmu.notes-nothink\endcsname{$-$1.0}
\expandafter\def\csname N@x.mmmu.notes-nothink.abs\endcsname{1.0}
\expandafter\def\csname N@x.mmmu.notes-nothink.ci\endcsname{[$-$4.2, +2.2]}
\expandafter\def\csname N@x.mmmu.notes-nothink.hi\endcsname{+2.2}
\expandafter\def\csname N@x.mmmu.notes-nothink.lo\endcsname{$-$4.2}
\expandafter\def\csname N@x.mmmu.notes-vanilla\endcsname{$-$2.5}
\expandafter\def\csname N@x.mmmu.notes-vanilla.abs\endcsname{2.5}
\expandafter\def\csname N@x.mmmu.notes-vanilla.ci\endcsname{[$-$5.2, +0.2]}
\expandafter\def\csname N@x.mmmu.notes-vanilla.hi\endcsname{+0.2}
\expandafter\def\csname N@x.mmmu.notes-vanilla.lo\endcsname{$-$5.2}
\expandafter\def\csname N@x.mmmu.notes-visible-vanilla\endcsname{$-$1.3}
\expandafter\def\csname N@x.mmmu.notes-visible-vanilla.abs\endcsname{1.3}
\expandafter\def\csname N@x.mmmu.notes-visible-vanilla.ci\endcsname{[$-$3.3, +1.0]}
\expandafter\def\csname N@x.mmmu.notes-visible-vanilla.hi\endcsname{+1.0}
\expandafter\def\csname N@x.mmmu.notes-visible-vanilla.lo\endcsname{$-$3.3}
\expandafter\def\csname N@x.mmmu.nothink-vanilla\endcsname{$-$1.5}
\expandafter\def\csname N@x.mmmu.nothink-vanilla.abs\endcsname{1.5}
\expandafter\def\csname N@x.mmmu.nothink-vanilla.ci\endcsname{[$-$4.7, +1.7]}
\expandafter\def\csname N@x.mmmu.nothink-vanilla.hi\endcsname{+1.7}
\expandafter\def\csname N@x.mmmu.nothink-vanilla.lo\endcsname{$-$4.7}
\expandafter\def\csname N@x.mmmu.pinsonly-vanilla\endcsname{$-$7.3}
\expandafter\def\csname N@x.mmmu.pinsonly-vanilla.abs\endcsname{7.3}
\expandafter\def\csname N@x.mmmu.pinsonly-vanilla.ci\endcsname{[$-$10.5, $-$4.3]}
\expandafter\def\csname N@x.mmmu.pinsonly-vanilla.hi\endcsname{$-$4.3}
\expandafter\def\csname N@x.mmmu.pinsonly-vanilla.lo\endcsname{$-$10.5}
\expandafter\def\csname N@x.mmmu.position-matched-vanilla\endcsname{$-$4.5}
\expandafter\def\csname N@x.mmmu.position-matched-vanilla.abs\endcsname{4.5}
\expandafter\def\csname N@x.mmmu.position-matched-vanilla.ci\endcsname{[$-$8.5, $-$0.5]}
\expandafter\def\csname N@x.mmmu.position-matched-vanilla.hi\endcsname{$-$0.5}
\expandafter\def\csname N@x.mmmu.position-matched-vanilla.lo\endcsname{$-$8.5}
\expandafter\def\csname N@x.vh.blind-vanilla\endcsname{$-$6.1}
\expandafter\def\csname N@x.vh.blind-vanilla.abs\endcsname{6.1}
\expandafter\def\csname N@x.vh.blind-vanilla.ci\endcsname{[$-$9.1, $-$3.1]}
\expandafter\def\csname N@x.vh.blind-vanilla.hi\endcsname{$-$3.1}
\expandafter\def\csname N@x.vh.blind-vanilla.lo\endcsname{$-$9.1}
\expandafter\def\csname N@x.vh.fixed-512-vanilla\endcsname{+0.4}
\expandafter\def\csname N@x.vh.fixed-512-vanilla.abs\endcsname{0.4}
\expandafter\def\csname N@x.vh.fixed-512-vanilla.ci\endcsname{[$-$1.8, +2.6]}
\expandafter\def\csname N@x.vh.fixed-512-vanilla.hi\endcsname{+2.6}
\expandafter\def\csname N@x.vh.fixed-512-vanilla.lo\endcsname{$-$1.8}
\expandafter\def\csname N@x.vh.notes-nothink\endcsname{$-$0.2}
\expandafter\def\csname N@x.vh.notes-nothink.abs\endcsname{0.2}
\expandafter\def\csname N@x.vh.notes-nothink.ci\endcsname{[$-$2.7, +2.4]}
\expandafter\def\csname N@x.vh.notes-nothink.hi\endcsname{+2.4}
\expandafter\def\csname N@x.vh.notes-nothink.lo\endcsname{$-$2.7}
\expandafter\def\csname N@x.vh.notes-vanilla\endcsname{$-$0.5}
\expandafter\def\csname N@x.vh.notes-vanilla.abs\endcsname{0.5}
\expandafter\def\csname N@x.vh.notes-vanilla.ci\endcsname{[$-$2.8, +1.8]}
\expandafter\def\csname N@x.vh.notes-vanilla.hi\endcsname{+1.8}
\expandafter\def\csname N@x.vh.notes-vanilla.lo\endcsname{$-$2.8}
\expandafter\def\csname N@x.vh.notes-visible-vanilla\endcsname{$-$1.5}
\expandafter\def\csname N@x.vh.notes-visible-vanilla.abs\endcsname{1.5}
\expandafter\def\csname N@x.vh.notes-visible-vanilla.ci\endcsname{[$-$3.8, +0.7]}
\expandafter\def\csname N@x.vh.notes-visible-vanilla.hi\endcsname{+0.7}
\expandafter\def\csname N@x.vh.notes-visible-vanilla.lo\endcsname{$-$3.8}
\expandafter\def\csname N@x.vh.nothink-vanilla\endcsname{$-$0.3}
\expandafter\def\csname N@x.vh.nothink-vanilla.abs\endcsname{0.3}
\expandafter\def\csname N@x.vh.nothink-vanilla.ci\endcsname{[$-$2.9, +2.3]}
\expandafter\def\csname N@x.vh.nothink-vanilla.hi\endcsname{+2.3}
\expandafter\def\csname N@x.vh.nothink-vanilla.lo\endcsname{$-$2.9}
\expandafter\def\csname N@x.vh.pinsonly-vanilla\endcsname{$-$4.4}
\expandafter\def\csname N@x.vh.pinsonly-vanilla.abs\endcsname{4.4}
\expandafter\def\csname N@x.vh.pinsonly-vanilla.ci\endcsname{[$-$6.7, $-$2.0]}
\expandafter\def\csname N@x.vh.pinsonly-vanilla.hi\endcsname{$-$2.0}
\expandafter\def\csname N@x.vh.pinsonly-vanilla.lo\endcsname{$-$6.7}
\expandafter\def\csname N@x.vh.position-matched-vanilla\endcsname{$-$4.2}
\expandafter\def\csname N@x.vh.position-matched-vanilla.abs\endcsname{4.2}
\expandafter\def\csname N@x.vh.position-matched-vanilla.ci\endcsname{[$-$6.4, $-$2.1]}
\expandafter\def\csname N@x.vh.position-matched-vanilla.hi\endcsname{$-$2.1}
\expandafter\def\csname N@x.vh.position-matched-vanilla.lo\endcsname{$-$6.4}
\newcommand{\N}[1]{\ifcsname N@#1\endcsname\csname N@#1\endcsname\else\PackageError{numbers}{Unknown number key #1}{}\fi}
\makeatother

